Enhancing Lidar Point Cloud Sampling via Colorization and Super-Resolution of Lidar Imagery

Recent advancements in lidar technology have led to improved point cloud resolution as well as the generation of 360 degrees, low-resolution images by encoding depth, reflectivity, or near-infrared light within each pixel. These images enable the application of deep learning (DL) approaches, originally developed for RGB images from cameras to lidar-only systems, eliminating other efforts, such as lidar-camera calibration. Compared with conventional RGB images, lidar imagery demonstrates greater robustness in adverse environmental conditions, such as low light and foggy weather. Moreover, the imaging capability addresses the challenges in environments where the geometric information in point clouds may be degraded, such as long corridors, and dense point clouds may be misleading, potentially leading to drift errors. Therefore, this paper proposes a novel framework that leverages DL-based colorization and super-resolution techniques on lidar imagery to extract reliable samples from lidar point clouds for odometry estimation. The enhanced lidar images, enriched with additional information, facilitate improved keypoint detection, which is subsequently employed for more effective point cloud downsampling. The proposed method enhances point cloud registration accuracy and mitigates mismatches arising from insufficient geometric information or misleading extra points. Experimental results indicate that our approach surpasses previous methods, achieving lower translation and rotation errors while using fewer points.

==> algs/al_kf.tex <==
\begin{algorithm}[t]
    \footnotesize
	\caption{UAV tracking fusing signal images and point clouds} 
	\label{alg:fusing_data}
	\KwIn{ \\
	    \vspace{.42em}
	    \hspace{.5em}Raw pointcloud:  $\mathcal{P}_{raw}^t$ \\
                  
	    \vspace{.23em}
	    \hspace{.5em}Signal image:  $\mathcal{S}^{t} $ \\

            \vspace{.23em}
	    \hspace{.5em}Target UAV point cloud:  $\mathcal{P}_{UAV}^{t-1}$ \\

	}
	\KwOut{  \\
	    \vspace{.42em}
	    \hspace{.5em}Drone pose: $\textbf{P}_{UAV}^{t}$\;
	    % \vspace{.23em}
        }
    \SetKwFunction{FMain}{object\_extraction}
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{\FMain{$\mathcal{P}_{raw}^t$, $\mathcal{P}_{UAV}^{t-1}$, $\mathcal{ROI}^t_{YOLO}$}}{
        \If{$\mathcal{ROI}^t_{YOLO}$}{
            $\mathcal{P}_{roi}^t$ = $\mathcal{P}_{raw}^t$ ($\mathcal{ROI}^t_{YOLO}$)\;
        }
        \Else{
            $\mathcal{ROI}^t \longleftarrow KF \left( get\_center\left( \mathcal{P}_{UAV}^{t-1} \right) \right)$\;
            
            % $\mathcal{P}_{roi}^t$ \longleftarrow\ $\mathcal{P}^t_{raw}$ ( $\mathcal{ROI}^{t}$)\;
        }
        $\mathcal{P}^t \longleftarrow ground\_removal\left( \mathcal{P}_{ROI}^t \right)$ \;
        $\mathcal{P}_{i}^t \longleftarrow DBSCAN \left( \mathcal{P}^t \right),\:i\in(0,R)$\;
        \ForEach{ $\mathcal{P}$ $\in$ $\mathcal{P}_{i}^t$ }{%
            \If{ Min (num($\mathcal{P}$ ) - num($\mathcal{P}_{UAV}^{t-1}$) )}{%
                \If{Min (dis($\mathcal{P}$) - dis($\mathcal{P}_{UAV}^{t-1}$))}{%
                    $flag = 1$ \;
                    $\mathcal{P}^{t}_{uav} \longleftarrow \mathcal{P}$ \;
                }
                
            \Else{
                $flag = 0$\;
                }
            }
            \Else{ 
                $flag = 0$\;}
        }
    \KwRet $\mathcal{P}_{uav}^{t}$, flag \;
    }
    \ForEach{ \textit{new} $\mathcal{S}^t$ }{
        $\mathcal{ROI}^t_{YOLO} \longleftarrow\ YOLOv5 \left( \mathcal{S}^{t} \right)$\;
        \If{$\mathcal{ROI}^t_{YOLO} = \textbf{None}$}{
            $\mathcal{P}_{UAV}^{t}$ , flag = \textit{object\_extraction} ($\mathcal{P}_{raw}^t$, $\mathcal{P}_{uav}^{t-1}$) \;
            \If{flag = 0}{
                $\textbf{P}_{UAV}^{t}$ = \textit{KF\_predict} (\textit{get\_center}($\mathcal{P}_{UAV}^{t-1}$))  \;
                \textit{KF\_update} ($\textbf{P}_{UAV}^{t}$)
            }
            \Else{
                $\textbf{P}_{UAV}^{t}$ = \textit{get\_center}($\mathcal{P}_{UAV}^{t}$)  \;
                \textit{KF\_update} ($\textbf{P}_{UAV}^{t}$)  \;
            }
        }
        \Else{
            $\mathcal{P}_{UAV}^{t} = object\_extraction \left( \mathcal{P}_{raw}^t, \:\mathcal{P}_{UAV}^{t-1}, \:\mathcal{ROI}^t \right)$ \;
            $\textbf{P}_{UAV}^{t} = get\_center \left(\mathcal{P}_{UAV}^{t} \right)$\;
            $KF\_update \left( \textbf{P}_{UAV}^{t} \right)$\;
        }
    }
\end{algorithm}



==> algs/evaluation-scheme.tex <==
\begin{algorithm}[h]
% \footnotesize
\DontPrintSemicolon
\SetNoFillComment
% \SetAlgoNoLine
    \caption{The evaluation scheme}
    \label{alg:eva-scheme}
    % \centering
    \KwIn{\\
        % \vspace{.42em}
	\hspace{1em} Range image: $rng$ \\
        % \hspace{1em} Signal image: $sig$ \\
        % \hspace{1em} Point cloud: $pc$ \\
        \hspace{1em} Combinations in Table~\ref{tab:combinations}: $\textit{combs} = [\textit{comb\_i}]$, $i\in(0\sim6) $
    }
    \BlankLine
    \KwOut{\\
        \hspace{1em} Translation error: \(trans\_err\;(mean/rmse, unit:\,m)\) \\
        \hspace{1em} Rotation error: \(rot\_err\;(mean/rmse, unit:\,^\circ)\) \\
    }
    \BlankLine

    \tcc{Variable Declarations:}
$Kp$ : Keypoint \\
$pc_{kp}$: Point Cloud Keypoint \\
% \textit{en\_img}: Enhanced image \\
\textit{LOC} : LiDAR Odometry Calculation \\
\textit{GT} : Ground Truth   \\

\vspace{0.23em}
    \tcc{Image preprocess for brighter images}
    \SetKwFunction{gamma}{gamma}
    \SetKwFunction{histequal}{hist\_equalizer}
    \SetKwFunction{FPreproc}{img\_preprocess}
    % \SetKwProg{Fn}{Function}{:}{}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FPreproc{$img$}}{
        % $img$ = {$sig$,$rng$}
        \If{$img$ == $rng$}{
            $img_{prc}$ $\gets$ \gamma($img$)\;
        }
        \Else{
            % \tcc{Keep pixels with a brightness greater than $p\_thresh$}
            \If{$pixel\_value < p\_thresh$}{     
                % \tcc{Adaptive Histogram Equalization Transform}
                $img\_hist$ $\gets$ \histequal($img$)\;     
                $img\_prc$ $\gets$ \gamma($img\_hist$)\;
                % $img\_{prc}$[$area\_w$] $\gets$ $img$[$area\_w$] \\    
                % }
                % mask = [$pixel\_value$ $\geq$ $p\_thresh$] \\
                % $area\_w$ = $img$[mask] \
            }
        }
        \KwRet $img\_{prc}$; 
        }
    \BlankLine
    \tcc{Key point detect & track}
    \SetKwFunction{MnnMatcher}{MnnMatcher}
    \SetKwFunction{FTracker}{kp\_detect\&track}
    \SetKwFunction{FColorization}{colorization}
    \SetKwFunction{FSuperresolution}{super\_resolution}
    \SetKwFunction{FKeypointdet}{keypoint\_detect}
    \SetKwProg{Fn}{def}{:}{}
    \Fn{\FTracker{\textit{img}, $kps_{t-1}$}}{
        % $pts_{t}$ $\gets$ round( $pts_{t}$ )\;
            % \tcc*[r]{Find matches using the MNN matcher in OpenCV}
            $kps_{t}$ $\gets$ \FKeypointdet(\textit{img}) \;
            $matches$ $\gets$ \MnnMatcher{$kps_{t-1}$, $kps_{t}$}\;
            mkps $\gets$ $kps_{t}$[$matches$]\;
            % mpts2 $\gets$ $kps_{t}$[$matches[:, 1]$]\;
            % N\_matches $\gets$ len(matches)\;
            % \tcc*[r]{Collect matched points coordinates}
            % current\_frame\_points $\gets$ \{(round(p2)) $\mid$ p2 $\in$ mpts2\}\;
        \KwRet{mkps}\;
    }
    \ForEach{$\textit{comb\_i}$ in $\textit{combs}$}{
    \tcc{In table\ref{tab:combinations},there are different $rng$ and $sig$ in comb}
        $rng$ = \FPreproc{$rng$}\;  
        $sig$ = \FPreproc{$sig$}\;
        \textbf{Perform} following process to every $rng$ in comb  \;
        \textit{en\_img} $\gets$ \FSuperresolution{$rng$}  \\
        % pts, desc $\gets$ \FKeypointdet(\textit{en\_img})\\
        $kp$ $\gets$ \FTracker{\textit{en\_img}, $kpts_{t-1}$}\\
        $pc_{kp}^{r}$ $\gets$ pc[index[$kp$]] \\
        \tcp*[h]{----------------------------------------------------}


        \textbf{Perform} following process to every \textbf{$sig$} in comb  \;
        
        % \If{$rng\_xt$ in \textit{comb\_i}}{
        %     $rng\_xt$ = \textit{super\_resolution($rng$)}\;
        % }
        
        % \If{$sig\_xt$ in \textit{comb\_i}}{
        %     $sig\_xt$ = \textit{super\_resolution($sig$)}\;
        %     If{ $sig\_xt_cl$ in \textit{comb\_i}}{
            
        %     }
        % }
        % \textit{img} $\gets$ \textit{Image preprocessing}($\textit{comb\_i}$) \\
        \textit{en\_img} $\gets$ \FSuperresolution{$sig$}  \\  
        \textit{en\_img} $\gets$ \FColorization{\textit{en\_img}}  \\
        % pts, desc $\gets$ \FKeypointdet\textit{en\_img})\\
        $kp$ $\gets$ \FTracker{\textit{en\_img}, $kpts_{t-1}$}\\
        $pc_{kp}^{s}$ $\gets$ pc[index[$kp$]] \\
        \tcp*[h]{----------------------------------------------------}
        $pc_{kp}$ $\gets$ integrate ($pc_{kp}^{r}$, $pc_{kp}^{s}$ )  \\
        % LO calculation with point cloud keypoint as input  \\
        Odom $\gets$ \textit{LOC}($pc_{kp}$) \\
        % Translation and rotation error computation \\
        \textit{trans\_err}, \textit{rot\_err} $\gets$ evo(Odom,GT) 
        \\
    }
\end{algorithm}

==> algs/pos_gd.tex <==


\begin{algorithm}[t]
    %
    %
    %
    \footnotesize
	\caption{\footnotesize Ground truth extraction}
	\label{alg:tracking}
	\KwIn{\\
	    \begin{tabular}{ll}
	        3D lidar point cloud:             & $\mathcal{P}$ \\
	        Last known MAV state:              & $ \textbf{p}^{k-1}_{MAV}, {\dot{\textbf{p}}_{MAV}}^{k-1}$ \\[+0.4em]
	    \end{tabular}
	}
	\KwOut{\\
	    \begin{tabular}{ll}
	        MAV state:      & \{${\textbf{p}^{k}_{MAV}}, \:\dot{\textbf{p}}^{k}_{MAV}\}$ \\[+0.2em] 
	    \end{tabular}
	}  
	%\BlankLine
	%
	\SetKwFunction{FSub}{$object\_extraction\left(\mathcal{P}, \:{\textbf{p}^{k-1}_{MAV}}, \:\dot{\textbf{p}}^{k-1}_{MAV}\right)$}
    \SetKwProg{Fn}{Function}{:}{}
    % Position estimation based on current PointCloud and last position and speed
    \BlankLine
%     \Fn{\FSub}
%     {
%             \vspace{.3em}
            
%             \KwRet ${\textbf{p}^{k}_{MAV}};$
%     }
% 	\BlankLine
    %
% 	$Adaptive\;Integrate\;Rate: I_{rate}$ \\
    % Calculate with high frequency, get the pose(high accuracy, but not robust)  
    % Coarse first, then fine grained estimate
    % \tcp{Coarse but persistent tracking}
    % \While{new $\mathcal{P}_{k}(I^{k}_{MF})$}{
    %     ${\textbf{p}^{k'}_{MAV}} =  object\_extraction(\mathcal{P}_{k}(I^{k}_{MF}), I^{k}_{MF}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
    %     % $Evaluate \; Estimation({\textbf{p}^{k-1}_{MAV}}, {\textbf{p}^{k}_{MAV}} )$ \\
    %     % $Update({\textbf{p}}^{k}, I_{rate} )$ \\
    % }
    % \tcp{Fine-grained estimation}
    \While{new $\mathcal{P}_{k}$}{
        \begin{tabular}{ll}
                Generate KD Tree:       & $kdtree \leftarrow \mathcal{P};$ \\
                MAV pos estimation:     & $\hat{\textbf{p}}_{\tiny MAV}^{k} \leftarrow \textbf{p}^{k-1}_{MAV} + \frac{\dot{\textbf{p}}_{MAV}^{k-1}}{I};$ \\[+0.4em]
                MAV points:             & $\mathcal{P}^{k}_{MAV} = KNN(kdtree, \: \hat{\textbf{p}}_{MAV}^{k});$ \\[+0.4em]
                MAV state estimation:   & ${\textbf{p}^{k}_{MAV}} = \frac{1}{\lvert\mathcal{P}^{k}_{MAV}\rvert}\sum_{p\in\mathcal{P}^{k}_{MAV}} p;$ \\
        \end{tabular}
        % ${\textbf{p}^{k''}_{MAV}} =  object\_extraction(\mathcal{P}_{k}, \textbf{p}^{k-1}_{MAV}, \dot{\textbf{p}}^{k-1}_{MAV});$ \\
        % ${\textbf{p}^{k}_{MAV}}, \: {\dot{\textbf{p}}^{k}_{MAV}} \leftarrow estimate\left(\textbf{p}^{k'}_{MAV}, \:\textbf{p}^{k''}_{MAV}\right)$\;
    }
    % $\{I^{k}_{HF}, I^{k}_{MF}\} \leftarrow adjust\_integration\_freqs\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$ \\[+0.4em]
    % $\dot{\textbf{q}}^{k}_{UGV} \leftarrow keep\_within\_FoV\left(\textbf{p}^{k}_{MAV}, \dot{\textbf{p}}^{k}_{MAV}\right);$
    
 
\end{algorithm}

==> sec/00_Abstract.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                                          %%
%%                ABSTRACT                  %%
%%                                          %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \IEEEtitleabstractindextext{%
% \fcolorbox{abstractbg}{abstractbg}{%
% \begin{minipage}{\textwidth}%
% \begin{wrapfigure}[13]{r}{0.42\textwidth}%
% % \includegraphics[width=0.4\textwidth]{fig/abstract-img.png}%
% \end{wrapfigure}%
\begin{abstract}%
    \label{sec:abstract}%
    Recent advancements in lidar technology have led to improved point cloud resolution as well as the generation of  360\textdegree\, low-resolution images by encoding depth, reflectivity, or near-infrared light within each pixel. 
    These images enable the application of deep learning (DL) approaches, originally developed for RGB images from cameras, to lidar-only systems, eliminating other efforts, such as lidar-camera calibration.   
    Moreover, the imaging capability addresses the challenges in environments where the geometric information in point clouds may be degraded, such as long corridors, and dense point clouds may be misleading, potentially leading to drift errors.

    Therefore, this paper proposes a novel framework that utilizes DL-based colorization and super-resolution techniques on lidar-generated images to extract reliable samples from lidar point clouds for odometry purposes.
    The colorization and super-resolution techniques are selected based on a concise review of conventional computer vision DL methods for image colorization and super-resolution, and the evaluation of performance on lidar-generated imagery conducted in this paper.
    The proposed method enhances point cloud registration accuracy and mitigates mismatches arising from insufficient geometric information or misleading extra points. Experimental results indicate that our approach surpasses previous methods, achieving lower translation and rotation errors while using fewer points.
\end{abstract}

\begin{IEEEkeywords}
    lidar, Odometry, Super-Resolution, Colorization,  lidar-as-a-camera, Point Cloud Sampling
\end{IEEEkeywords}
% \end{minipage}}}

==> tbs/list-colorization.tex <==
\begin{table*}[t]
    \centering
    \caption{ Details of Deep Learning-based Colorization Models } 
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccclc}
    \hline
    \textbf{Model} & \textbf{Indoor} & \textbf{Outdoor} & \textbf{Code} & \textbf{Description} & \textbf{Language compatible}\\ \hline
    \textit{DeOldify~\cite{antic2019deoldify}} & $\surd$ & $\surd$ & $\surd$ & Effectiveness in restoring and colorizing old black-and-white photos & Python3 \\
    \textit{DDColor~\cite{kang2023ddcolor}} & $\surd$ & $\surd$ & $\surd$ & Utilizes diffusion models for high-quality image colorization & Python3 \\
    \textit{BigColor~\cite{kim2022bigcolor}} & $\surd$ & $\surd$ & $\surd$ & Designed for large-scale, high-resolution image colorization & Python3 \\ 
    \textit{BigGAN~\cite{brock2018large}} & & $\surd$ & & Generating high-resolution, high-fidelity natural images \\
    \textit{PearlGAN~\cite{luo2022thermal}} &  & $\surd$ & $\surd$ & Focuses on colorizing thermal and infrared images using GANs, effective in outdoor environments & Python3\\
    \textit{I2V-GAN~\cite{I2V-GAN2021}} &  & $\surd$ & $\surd$ & GAN-based model for colorizing infrared to visible spectrum images & Python3\\
    \textit{Colorful Image Colorization~\cite{zhang2016colorful, zhang2017real}} & $\surd$ & $\surd$ & $\surd$ & One of the first CNN-based colorization models, introducing probabilistic color assignment & Python3\\
    \textit{Let there be Color~\cite{IizukaSIGGRAPH2016}} & $\surd$ & $\surd$ & $\surd$ & A fully automatic image colorization method that works on both grayscale and natural images using deep learning & Lua\\
    \textit{DISCO~\cite{XiaHWW22}} & $\surd$ & $\surd$ & $\surd$ & Uses deep neural networks to provide automatic colorization with a focus on preserving detail and texture & Python3\\ 
    \textit{Deep Koalarization~\cite{DBLP:journals/corr/abs-1712-03400}} & $\surd$ & $\surd$ & $\surd$ & Combines a pre-trained VGG network with a colorization model for realistic colorization & Python3\\ 
    \textit{Palette~\cite{paltte}} & $\surd$ & $\surd$ & $\surd$ & A versatile colorization model that leverages palette-based techniques to achieve high-quality results across various image types & Python3\\
    \textit{ChromaGAN~\cite{vitoria2020chromagan}} & $\surd$ & $\surd$ & $\surd$ & GAN-based model that emphasizes perceptual loss for natural colorization results & Python3\\ 
    \textit{InstColorization~\cite{Su-CVPR-2020}} & $\surd$ & $\surd$ & $\surd$ & An instance-aware colorization model that handles complex scenes by focusing on individual object instance & Python3\\
    \textit{SCGAN~\cite{zhao2020scgan}} & $\surd$ & $\surd$ & $\surd$ & A self-consistent GAN-based colorization approach that ensures color consistency across different regions of an image & Python3\\
    \textit{pix2pix~\cite{pix2pix2017}} & $\surd$ & $\surd$ & $\surd$ & A general-purpose image-to-image translation model & Python3\\ \hline
    \end{tabular}
    }
    \label{tab:colorization_models}   
\end{table*}





==> tbs/list-super-resolution.tex <==
\begin{table*}[t]
    \centering
    \caption{ Details of Deep Learning based Super Resolution Models } 
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lcllllc}
    \toprule
    \textbf{Model} & \textbf{Code} & \textbf{Architecture} & \textbf{Training Data} & \textbf{Strengths} & \textbf{Weaknesses} & \textbf{Language compatible} \\ 
    \midrule
    \textit{SRCNN~\cite{dong2015image}} &  & 3-layer CNN & ImageNet & Simple, Effective & Limited long-range dependency capture \\
    \textit{VDSR~\cite{kim2016accurate}} &  & 20-layer CNN & ImageNet & Deep architecture, Residual learning & High computational cost \\
    \textit{SRGAN~\cite{ledig2017photo}} &  & CNN with GAN & ImageNet, DIV2K & High perceptual quality & Potential artifacts \\
    \textit{DRRN~\cite{Tai-DRRN-2017}} &  & Recursive Residual Network & ImageNet, DIV2K & Parameter efficient, Deep architecture & High computational cost \\
    \textit{CARN~\cite{ahn2018fast}} & $\surd$ & Cascading Residual Network & DIV2K & Lightweight, Fast inference & Slightly lower accuracy & Python3\\
    \textit{SwinIR~\cite{liang2021swinir}} & $\surd$ & Transformer-based & DIV2K, Flicker2K & High performance, Handles large scale factors & High computational cost & Python3 \\  
    \textit{SCUNet~\cite{zhang2023practical}} & $\surd$ & CNN with Spatially Consistent Normalization & DIV2K & Maintains spatial consistency, Effective edge preservation & High computational resources, Training complexity & Python3 \\ 
    \textit{ESRGAN~\cite{wang2018esrgan}} & $\surd$ & GAN with Residual-in-Residual Dense Blocks & DIV2K, Flicker2K & Realistic textures, Superior perceptual quality & High computational cost, Can produce artifacts & Python3 \\ 
    \textit{DCSCN~\cite{yamanaka2020fastaccurateimagesuper}} & $\surd$ & CNN and Sparse Coding & CIFAR-10, ImageNet & Efficient high frequency detail capture & Struggles with complex images & Python3 \\ 
    \textit{RGT~\cite{chen2024recursive}} & $\surd$ & Recursive Generation Transformer & DIV2K, Flickr2K & Excellent handling of recursive structures & High computational demands & Python3 \\
    \textit{CAT~\cite{chen2022cross}} & $\surd$ & Cross-Attention Transformer & DIV2K, Flickr2K & Strong cross-modal learning, High fidelity & Computationally expensive & Python3 \\
    \textit{Perceptual Losses~\cite{johnson2016perceptual}} &  & CNN with Perceptual Loss & MS-COCO, ImageNet & High-quality image generation, Real-time performance & Dependent on pre-trained networks, Generalization limits\\ 
    \textit{SinGAN~\cite{rottshaham2019singan}} & $\surd$ & GAN with Single Image Learning & Single Image & Effective for artistic enhancement, Versatile & Training on each image required, Limited scalability & Python3 \\ 
    \textit{DnCNN~\cite{zhang2017beyond, zhang2020plug}} & $\surd$ & Deep CNN with Batch Normalization & ImageNet, BSD400 & Effective denoising, Simple architecture & Limited to small scale factors & Python3 \\ 
    \textit{SR3~\cite{9887996}} & $\surd$ & Diffusion Model for SR & CelebA-HQ, FFHQ & Generates realistic and high-quality images & High computational cost, Slow inference & Python3 \\
    \textit{EDSR~\cite{Lim_2017_CVPR_Workshops}} &  & Enhanced Deep Residual Network & DIV2K & High accuracy, No batch normalization & Requires extensive training, Large memory footprint \\ 
    \bottomrule
    \end{tabular}
    }
    \label{tab:sr_models} 
\end{table*}




==> tbs/result-colorization.tex <==
\begin{table}[h]
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{@{}llcc@{}}
    \toprule
    \textbf{Model}           & \textbf{Input size}  & \textbf{Output size} & \textbf{Running speed (secs/image)} \\ 
    \midrule
    BigColor                    & (1024, 128) & (1024, 128) & 0.54 \\
    Colorful Image Colorization & (1024, 128) & (1024, 128) & 0.27 \\ 
    DDColor                     & (1024, 128) & (1024, 128) & 0.37 \\ 
    DeOldify                    & (1024, 128) & (1024, 128) & 0.23 \\
    DISCO                       & (1024, 128) & (1024, 128) & 3.27 \\
    InstColorization            & (1024, 128) & (256, 256)  & 0.05 \\
    PearlGAN                    & (1024, 128) & (1024, 128) & 0.28 \\ 
    \bottomrule
    \end{tabular}
}
    \caption{Comparison of running speed of each colorization model based on local environment}
    \label{tab:color_speed}
\end{table}



==> tbs/result-sr.tex <==
\begin{table}[h]
\resizebox{0.48\textwidth}{!}{%
    \begin{tabular}{@{}llcc@{}}
    \toprule
    \textbf{Model}  & \textbf{Input size}  & \textbf{Output size} & \textbf{Running speed (secs/image)}  \\ \midrule
    CARN   & (1024, 128) & (2048, 256) & 0.005 \\
    SwinIR & (1024, 128) & (4096, 512) & 2.217 \\ 
    DCSCN  & (1024, 128) & (2048, 256) & 0.238 \\ 
    ESRGAN & (1024, 128) & (4096, 512) & 2.667 \\
    SCUNET & (1024, 128) & (1024, 128) & 1.706 \\ \bottomrule
    \end{tabular}
}
    \caption{Comparison of running speed of each super-resolution model based on local environment}
    \label{tab:color_speed}
\end{table}


==> tex/XYZ_plot/XY_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(1.35,1.00)},
  anchor=south east,
  draw=white,
  /tikz/every even column/.append style={column sep=0.5cm},
},
legend columns=3,
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
        minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.2937600641077, xmax=4.02480477083426,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=2.12877276002231, ymax=5.16023554096054,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.73259080042564 2.2954216427211
2.74343163560815 2.31777733333452
2.76226672899973 2.33763132237825
2.77197038543539 2.37099891932597
2.77941772327846 2.39915270681096
2.78829972509503 2.43237971210357
2.79987289003186 2.48228843678183
2.81119314984344 2.50723591521166
2.80290796777034 2.57016757457341
2.79863298401608 2.61110224606921
2.77857855552648 2.65472841443386
2.76879705733064 2.69645540690029
2.75941210404591 2.73302168382298
2.73673221300456 2.78460398196515
2.72048243208293 2.83162000452564
2.70981135271734 2.87356750945619
2.70740219155114 2.92110874032325
2.72064163397116 2.97777074365821
2.74227311431043 3.02254324868717
2.76767565170557 3.09168373521269
2.79776355687598 3.13921476015578
2.84619489817872 3.20421169494298
2.87781080242177 3.26403626073103
2.91866555366626 3.308839878853
2.95885920391216 3.35316934072594
2.99111507738432 3.39633428969372
3.01853055180776 3.43829247711476
3.04301459264569 3.47959461117091
3.07663927060839 3.50625344126635
3.11054872763804 3.52119343091084
3.12983829173943 3.55705093628962
3.17180958828291 3.58359333367066
3.22576927251157 3.61456898100191
3.28173252084285 3.66382379414986
3.33522348003846 3.70350267599603
3.38826456094178 3.73986772656383
3.42938132912533 3.79459211832735
3.47478516109619 3.8589167167674
3.49920348070984 3.92124063459251
3.51926711555732 3.99992257838136
3.53323378630256 4.04932519277265
3.5104876649043 4.12635767857896
3.50924029339517 4.18267360064715
3.49381577645071 4.26760867678425
3.46585263690297 4.33154077984819
3.42616129615141 4.40008314812554
3.39381158144173 4.44440381051309
3.35878389826143 4.50073852441353
3.31842252627628 4.54387388862518
3.28373377124474 4.57784565316582
3.26717255524395 4.61861403199193
3.20625048331003 4.65154330276112
3.14292769800767 4.64713122150596
3.10984578909261 4.65879743126192
3.03028290664255 4.70050728512957
2.98342308024528 4.71491058954871
2.90833750529192 4.66791998111957
2.81369016358825 4.66456338564272
2.68960518051834 4.6514615485341
2.61834317180246 4.61419404518564
2.59133359628131 4.57197420706711
2.53889867078703 4.53758470508788
2.49640102134837 4.46912709671841
2.43093337475764 4.42916135383894
2.41406072727463 4.34431157821041
2.38916320019083 4.25510880352394
2.38424727687088 4.19943957942588
2.3797065920442 4.10868519659685
2.3804940506239 4.03084815122655
2.38711249426717 3.96403028690104
2.38454997523936 3.87862436703802
2.38524487352131 3.81631763394191
2.4086064252633 3.75911789075354
2.44214202121798 3.71140899378346
2.47419208213707 3.65434881455194
2.52827375525438 3.60680009805964
2.59370041123844 3.58652056216466
2.64731952288101 3.55043822523879
2.73361202424747 3.53340288012352
2.81427216858312 3.52469800454746
2.90816328526587 3.52613146215501
2.96942244815454 3.50699401464921
3.04041606903737 3.54187917205913
3.08431936930925 3.53992240245697
3.13378486714116 3.55999978636447
3.15156481646775 3.58142860940515
3.19113576408744 3.59744380239372
3.20853207243552 3.61509018467778
3.22592080248474 3.64513837855198
3.24157625200172 3.67737153279367
3.26849122905683 3.70888977791336
3.29794225893743 3.76111119411413
3.34512934296052 3.81567450582051
3.3871017149695 3.87873492581653
3.44399595481758 3.94845073923546
3.50091762439694 4.00428374323119
3.55147346702835 4.07382113314224
3.58816732015563 4.13568268890664
3.61049923891057 4.22094809638009
3.60773687233267 4.28045051725409
3.60600726786476 4.35828816630771
3.55194239633667 4.4285547032453
3.51784149259861 4.47791919068106
3.43165381383551 4.55688852191186
3.36386457197198 4.62122417091992
3.29561769526148 4.68121848605205
3.24881431706591 4.73146398329164
3.20861244380214 4.78350441257105
3.16938767019224 4.83617557570634
3.18050056208889 4.88170283359478
3.16503509773993 4.93427000544225
3.208614253057 4.95618168663791
3.18412356131201 4.95904613541331
3.21190362926877 4.97156268814394
3.21027400805481 4.96111937046137
3.1700639722792 4.95360187519411
3.11517225580331 4.94110527615339
3.07335484285838 4.90874431955096
2.99570056124122 4.88445928190409
2.85846299112991 4.84402526283237
2.78757485262802 4.81363791051145
2.74221472731354 4.74639621909141
2.63435390947082 4.70270904061743
2.56660606991018 4.64008299046569
2.51794481030488 4.57376563144212
2.46911614289648 4.49753014236375
2.45058709697382 4.4323391667904
2.47135825381675 4.3752508721595
2.45283485458011 4.30350269834918
2.49496367430251 4.23780888271187
2.48904701255822 4.16120874459902
2.5646343025954 4.08395576213948
2.5687428966418 3.99330635987506
2.58730541323742 3.90717893497241
2.62251700243816 3.82396238528935
2.64333416476756 3.73051040945206
2.67948897550178 3.67380135412162
2.72166591565624 3.62732310185697
2.75270055594358 3.60816445200711
2.80677818151326 3.6098946166593
2.85133018420882 3.62974614417943
2.91066751505617 3.63564250016771
2.98482763034345 3.67777015015346
3.06730554673034 3.71591579123588
3.14460274091814 3.75898147583426
3.23213784635088 3.79552346889038
3.31024163079453 3.82217176546725
3.3512951091394 3.85307696350958
3.4017711046021 3.88682844445628
3.38549056476237 3.88813003946867
3.40526244113241 3.89499281734444
3.40346612365705 3.89927045065691
3.39371821855194 3.86211921707423
3.4019140630963 3.8675035459905
3.43280327400255 3.8550389843343
3.42039131920034 3.84582553031054
3.47478814252454 3.82192860675603
3.52481279222092 3.8188104365502
3.59465430557435 3.81326090765918
3.64292121266644 3.79713954466694
3.71732876891936 3.77813464376112
3.78228755694404 3.76760799931913
3.84326397997338 3.73444576200688
3.87591104971136 3.70009956408722
3.90045321168651 3.64725299707619
3.91996780654539 3.57459200766659
3.89384541236475 3.49507137704457
3.8532622045896 3.40462543050264
3.8009317601632 3.31878053771735
3.747730859615 3.21306244747252
3.66707106515983 3.11988218513941
3.5915272141181 3.03607055697764
3.52093959907854 2.95875103539358
3.45350962038186 2.90943214434925
};
\addlegendentry{Ours }
\addplot [line width=1pt, color0]
table {%
2.73138986085617 2.26656652279223
2.75360432320259 2.35714382130048
2.7508083515257 2.46912835587662
2.74550851348316 2.54904439484317
2.72250258307611 2.61610617873149
2.70890036336189 2.67091839597072
2.70048674867281 2.71293841304514
2.6621245905157 2.8289300166783
2.65258940451437 2.8774984141375
2.65388347721636 2.9297412196155
2.67367372667819 2.99582687673874
2.71430448120537 3.04398971125765
2.75246716597602 3.11821334733149
2.86294371432932 3.23500900778058
2.90622962533318 3.29710121648793
2.95056109235385 3.34523716767429
2.99364341688218 3.38133012793502
3.02859427991752 3.42218117361351
3.05303250126545 3.46468232077013
3.07371619488321 3.50232048035524
3.13888316455779 3.53138675226301
3.16026821946876 3.56050365837881
3.2011036391208 3.5866636872793
3.26194031975455 3.61679437274807
3.324686196072 3.66508438167831
3.39168199789358 3.71110243709038
3.45507064740115 3.74881729731915
3.54791406710348 3.87321212722207
3.56893738355065 3.94332451694098
3.57555290050113 4.02933308877975
3.58155283205009 4.09019776487595
3.54932629113885 4.16508434190537
3.53567629037423 4.22440220256894
3.51997284555271 4.30491172300629
3.433437696447 4.45110679138145
3.39377508547388 4.49818151091311
3.35114383424233 4.54490620065661
3.31313908978661 4.58474715181891
3.28820382358359 4.61732776598191
3.27425116100906 4.64513056496436
3.21557335445532 4.68209119320882
3.09517642619145 4.67689255581475
3.0237912725378 4.71121890184527
2.96730721438741 4.72908747193449
2.88654480121457 4.68988240652772
2.7825827012005 4.67061365107596
2.66926498137833 4.66318354414061
2.56055966975768 4.62011394913901
2.49794002158032 4.52897023159987
2.46771011458673 4.45192419369431
2.41016471761844 4.40100904910164
2.38746546621496 4.31615609623814
2.38373945569784 4.22276895453488
2.37568340169178 4.1513383273049
2.37438529736967 4.06132088987714
2.39164826922535 3.91240201883462
2.3902769834158 3.83365064700832
2.38948524431167 3.76827987219866
2.40738441948655 3.71381407610171
2.45310103488526 3.67536896327288
2.49340311007651 3.62523566406642
2.55163154853127 3.57816940186485
2.69675335918421 3.53342552792813
2.7828881224921 3.51982087848909
2.8781491291644 3.51785614866331
2.97401096266729 3.52830366103386
3.04490491628471 3.51297702842778
3.10674838697937 3.54607893560372
3.14268939458707 3.56705205771726
3.19304735985892 3.60401281076548
3.21979241206349 3.62928634441175
3.23261212494025 3.64446115856433
3.24157911978149 3.67286715948425
3.25282331608796 3.71002245775272
3.27531500357294 3.74868867147703
3.30946525165874 3.80102292687833
3.42385911017909 3.93236281040655
3.4925721935755 4.00647533265346
3.55868134397623 4.06658877149959
3.62211398508616 4.13244637976297
3.65590555658562 4.1961475001081
3.66762449416404 4.27739257805573
3.65635034189895 4.34797240131824
3.57450225759951 4.49815402389132
3.5158561928853 4.55318674767089
3.41539104845262 4.63109920128498
3.33620951102076 4.70003778680557
3.25981144745224 4.76173411000382
3.21774691837508 4.80983644276065
3.18190880196593 4.85795678179988
3.17415752571927 4.94957756098052
3.17693561005654 5.00200282074395
3.22823553566057 5.02244177819062
3.23357894433589 5.01361867542625
3.25220577008086 5.01083580216477
3.2515280013004 4.99080038985157
3.20585824063552 4.97426244268442
3.06770239653192 4.92098387821703
2.97668730023826 4.89068955830255
2.84576909514051 4.85105684806315
2.72324522445048 4.81949275852938
2.66511587162346 4.75215494766644
2.56737987444208 4.7000965492915
2.49471329396189 4.6370482848981
2.4093239167304 4.48600491487912
2.39956970376416 4.4143954307876
2.4376903406125 4.35508778149186
2.44608059076592 4.28856147136882
2.49113634814668 4.21924292669192
2.49765126578515 4.14232480811796
2.57138202453032 4.05807420954335
2.60142040165522 3.87004989365037
2.63148326539495 3.78420504498652
2.65489646110252 3.69286429381683
2.67590307732644 3.63283440896259
2.71555056669599 3.60052766507381
2.75553028398983 3.59385470673663
2.80934333571462 3.61573660602321
2.92733741621492 3.67854550142618
3.00795400936487 3.72883539212453
3.113924435822 3.78066445016795
3.20209421874616 3.82685738124627
3.29513009591462 3.86869615050429
3.37406738163484 3.89120954533684
3.41678144100867 3.91382799082125
3.42748138373125 3.9365317018496
3.41629296783595 3.93210645408647
3.39991136029194 3.93231502623131
3.38655207560852 3.89157036167549
3.38100526590359 3.87612959104443
3.41160372311744 3.86039258272765
3.42411932536854 3.84920205010396
3.46911867279182 3.82223804415004
3.62774585499471 3.81118702895529
3.68700583597362 3.78918835850452
3.76279959859637 3.76273740012428
3.83677982126538 3.74379930250183
3.89950867841041 3.71244778006224
3.93350333458381 3.66098633321622
3.94612092052851 3.51781356500873
3.90038448028181 3.42482929034603
3.83280522309102 3.32435618429358
3.75225049030137 3.22850809599341
3.67462506650057 3.12001769870334
3.57868141193329 3.02508054511676
3.48884590654207 2.9409249519996
3.33868769525814 2.83436894351627
3.27961156151381 2.79343853460443
3.24219519876619 2.76691028471854
};
\addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.79194092027163 2.35892892452518
% 2.79407119406988 2.42978630582589
% 2.79527527534208 2.48453329989567
% 2.79418461279521 2.53544276599431
% 2.7992917117979 2.60163917930246
% 2.81102871558341 2.63961579753378
% 2.79760860772589 2.70738974953776
% 2.78645569767935 2.75855673276656
% 2.75987040227934 2.8035775783111
% 2.74492820427677 2.84376380208128
% 2.73700166567946 2.8750528381069
% 2.71236227704775 2.92158934911775
% 2.68765841775157 2.97520109740467
% 2.67290493528827 3.02040086164092
% 2.66640708423765 3.06965739993503
% 2.67907644603627 3.13503458401981
% 2.71122620765581 3.1852448045617
% 2.73898108045827 3.26139294599305
% 2.78053817349636 3.31810043051243
% 2.83576546128013 3.38685611116533
% 2.86746986064176 3.45422213542551
% 2.90443960573929 3.50698442114095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.78004336357117 2.44961881637573
2.78473997116089 2.49184632301331
2.78169870376587 2.53642201423645
2.77279257774353 2.5811128616333
2.7611358165741 2.62548923492432
2.74732780456543 2.66858124732971
2.73093748092651 2.71244502067566
2.69390487670898 2.80324053764343
2.68285369873047 2.84974360466003
2.68129086494446 2.89853239059448
2.68994092941284 2.95167922973633
2.7073175907135 3.00733399391174
2.73254680633545 3.06419110298157
2.80578780174255 3.17853021621704
2.84787058830261 3.23518180847168
2.89023494720459 3.28984522819519
2.9271776676178 3.34109807014465
2.96092367172241 3.38540554046631
2.99176788330078 3.42358613014221
3.02260088920593 3.4562566280365
3.08351445198059 3.50875163078308
3.11538076400757 3.53420877456665
3.15450525283813 3.55867266654968
3.20232772827148 3.58785653114319
3.25803208351135 3.6181046962738
3.3161768913269 3.65492224693298
3.37219643592834 3.70083785057068
3.47152757644653 3.80997467041016
3.50878357887268 3.87289643287659
3.53404450416565 3.93877172470093
3.54474639892578 4.00425100326538
3.54177737236023 4.07564973831177
3.5278651714325 4.14390993118286
3.50693893432617 4.21157598495483
3.44325828552246 4.34743690490723
3.41175317764282 4.3992977142334
3.38133764266968 4.44696283340454
3.34080910682678 4.50991916656494
3.31128025054932 4.55272197723389
3.27819752693176 4.59152603149414
3.23718738555908 4.62049102783203
3.13333964347839 4.66143894195557
3.0713849067688 4.67684459686279
3.00010514259338 4.68613862991333
2.93614459037781 4.68156385421753
2.84673571586609 4.67292547225952
2.7660768032074 4.65167999267578
2.68826532363892 4.62711381912231
2.56908178329468 4.56195640563965
2.4967725276947 4.48921155929565
2.45544767379761 4.42907476425171
2.42531800270081 4.364417552948
2.39972305297852 4.28832912445068
2.38822770118713 4.21258687973022
2.38112616539001 4.13534498214722
2.37244391441345 3.9815731048584
2.37436366081238 3.91040086746216
2.38197445869446 3.84459114074707
2.38410639762878 3.83271741867065
2.38410639762878 3.83271741867065
2.54188394546509 3.59143424034119
2.54188394546509 3.59143424034119
2.63489747047424 3.55322051048279
2.71523118019104 3.53378105163574
2.79587984085083 3.52052617073059
2.87371587753296 3.51484632492065
2.94537568092346 3.51649236679077
3.00989937782288 3.52600789070129
3.02894711494446 3.53686928749084
3.1410870552063 3.56351637840271
3.16888523101807 3.57629799842834
3.19266724586487 3.59665036201477
3.21331095695496 3.62381148338318
3.23522543907166 3.65565609931946
3.25612902641296 3.696049451828
3.28694272041321 3.73732781410217
3.37403917312622 3.84776592254639
3.43747353553772 3.91309595108032
3.46730494499207 3.94392347335815
3.54685282707214 4.03354120254517
3.56150364875793 4.05302429199219
3.56150364875793 4.05302429199219
3.55420994758606 4.41191577911377
3.55420994758606 4.41191577911377
3.52897119522095 4.44498062133789
3.46123027801514 4.51591968536377
3.44793391227722 4.52946996688843
3.44793391227722 4.52946996688843
3.20479941368103 4.8422794342041
3.20479941368103 4.8422794342041
3.20333743095398 4.84621095657349
3.19610905647278 4.88337802886963
3.20433259010315 4.92765474319458
3.20877623558044 4.93645238876343
3.20877623558044 4.93645238876343
3.10875654220581 4.93231248855591
3.10875654220581 4.93231248855591
3.09200954437256 4.92480373382568
3.0337131023407 4.9000825881958
2.81984186172485 4.80996656417847
2.81984186172485 4.80996656417847
2.74672770500183 4.77510261535645
2.66049242019653 4.72225284576416
2.59113669395447 4.67178773880005
2.47602367401123 4.53933477401733
2.44892525672913 4.4741735458374
2.44124889373779 4.4066367149353
2.44737863540649 4.33526086807251
2.46477293968201 4.2646312713623
2.48559141159058 4.19270467758179
2.5109715461731 4.11613798141479
2.56022667884827 3.95782518386841
2.59123277664185 3.86118698120117
2.61795139312744 3.78020834922791
2.64434695243835 3.71509742736816
2.67542433738708 3.66681861877441
2.7141900062561 3.63695573806763
2.75917601585388 3.62501287460327
2.87690043449402 3.65587210655212
2.94824028015137 3.68864607810974
3.02909922599792 3.72396874427795
3.1125910282135 3.75977635383606
3.19374990463257 3.79366683959961
3.25704741477966 3.82296109199524
3.32147431373596 3.85447812080383
3.3886239528656 3.89113712310791
3.3969361782074 3.89532256126404
3.39630007743835 3.89313435554504
3.3953697681427 3.88669848442078
3.39798903465271 3.8734872341156
3.4073429107666 3.85793447494507
3.42936635017395 3.84170961380005
3.45953583717346 3.82747554779053
3.5581591129303 3.80352425575256
3.62155294418335 3.7911856174469
3.69111347198486 3.77538084983826
3.76070165634155 3.75537896156311
3.82333898544312 3.72709131240845
3.86648988723755 3.69070506095886
3.91346454620361 3.56822967529297
3.89978837966919 3.49198365211487
3.86199855804443 3.40586566925049
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
3.81219482421875 3.32272267341614
};
\addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/XYZ_plot/XZ_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
            minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.2937600641077, xmax=4.02480477083426,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.404950771684837, ymax=1.54912152663555,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.73259080042564 0.456958533273505
2.74343163560815 0.49487950715315
2.76226672899973 0.529290846679961
2.77197038543539 0.558159603164172
2.77941772327846 0.581603031021609
2.78829972509503 0.611786834903712
2.79987289003186 0.619828840130322
2.81119314984344 0.618996725006725
2.80290796777034 0.628498933188615
2.79863298401608 0.618617386776924
2.77857855552648 0.614607834975727
2.76879705733064 0.595761471537237
2.75941210404591 0.587547656728352
2.73673221300456 0.590958649413665
2.72048243208293 0.591881436489796
2.70981135271734 0.587976674053637
2.70740219155114 0.602002696201986
2.72064163397116 0.60076945794349
2.74227311431043 0.599485724584289
2.76767565170557 0.606668274298737
2.79776355687598 0.601798888398763
2.84619489817872 0.601803934405946
2.87781080242177 0.624994661038883
2.91866555366626 0.618054264314445
2.95885920391216 0.633184133508421
2.99111507738432 0.621581680741958
3.01853055180776 0.608653774943656
3.04301459264569 0.575099462250055
3.07663927060839 0.572568446543079
3.11054872763804 0.572684579097422
3.12983829173943 0.582454008587114
3.17180958828291 0.572830630436128
3.22576927251157 0.57180452551432
3.28173252084285 0.591655611703931
3.33522348003846 0.601012115979793
3.38826456094178 0.597981792655272
3.42938132912533 0.583684884156747
3.47478516109619 0.588966843957799
3.49920348070984 0.59836364931814
3.51926711555732 0.597582087944079
3.53323378630256 0.593434769797821
3.5104876649043 0.595421832362148
3.50924029339517 0.587168678823642
3.49381577645071 0.61323269863585
3.46585263690297 0.619632582003686
3.42616129615141 0.616422580950774
3.39381158144173 0.642036095741194
3.35878389826143 0.627756915178666
3.31842252627628 0.600471148141839
3.28373377124474 0.616949772980762
3.26717255524395 0.638238638834733
3.20625048331003 0.644806702267674
3.14292769800767 0.63367921735363
3.10984578909261 0.669634341593406
3.03028290664255 0.689264916110825
2.98342308024528 0.670265382912131
2.90833750529192 0.673432023045431
2.81369016358825 0.663546258504555
2.68960518051834 0.673433980979231
2.61834317180246 0.658970398827948
2.59133359628131 0.666703837043153
2.53889867078703 0.671934417412527
2.49640102134837 0.653844414067499
2.43093337475764 0.65968524912859
2.41406072727463 0.685358084016413
2.38916320019083 0.69307586205989
2.38424727687088 0.701937000010989
2.3797065920442 0.720095622449483
2.3804940506239 0.724435974931953
2.38711249426717 0.731778433289824
2.38454997523936 0.741309372872078
2.38524487352131 0.734836655091209
2.4086064252633 0.761445802916635
2.44214202121798 0.759670298112906
2.47419208213707 0.789383693822738
2.52827375525438 0.803059543989636
2.59370041123844 0.813322396882952
2.64731952288101 0.824897819019936
2.73361202424747 0.840585453207842
2.81427216858312 0.849309565324545
2.90816328526587 0.879255694390182
2.96942244815454 0.87885509882795
3.04041606903737 0.904607260521757
3.08431936930925 0.911776331357928
3.13378486714116 0.926187070720048
3.15156481646775 0.934689504021621
3.19113576408744 0.933546064274718
3.20853207243552 0.954467023878263
3.22592080248474 0.966678058414332
3.24157625200172 0.956835685894477
3.26849122905683 0.973457766206282
3.29794225893743 0.976457955699481
3.34512934296052 0.978880187295118
3.3871017149695 0.978734109121055
3.44399595481758 0.96995812975022
3.50091762439694 0.97968247290656
3.55147346702835 0.964835905435578
3.58816732015563 0.963451033157929
3.61049923891057 0.995157931634678
3.60773687233267 0.972477292621147
3.60600726786476 0.951715788645927
3.55194239633667 0.95058415575198
3.51784149259861 0.960707664166411
3.43165381383551 0.984419651304546
3.36386457197198 0.971751831612376
3.29561769526148 0.985980195289496
3.24881431706591 1.00240644796764
3.20861244380214 1.01293429952561
3.16938767019224 1.02839853580769
3.18050056208889 1.05042831139707
3.16503509773993 1.08165869271809
3.208614253057 1.1164418127072
3.18412356131201 1.10544999991501
3.21190362926877 1.14284870029486
3.21027400805481 1.13248620425793
3.1700639722792 1.12856981396099
3.11517225580331 1.12136826430779
3.07335484285838 1.13975526380678
2.99570056124122 1.15118368116767
2.85846299112991 1.19951970322011
2.78757485262802 1.20221132249522
2.74221472731354 1.20186365755875
2.63435390947082 1.21033719632458
2.56660606991018 1.21925373592581
2.51794481030488 1.22002153597137
2.46911614289648 1.23972725018781
2.45058709697382 1.25168273938092
2.47135825381675 1.23057699533913
2.45283485458011 1.25793334385766
2.49496367430251 1.23861195945078
2.48904701255822 1.25862519873877
2.5646343025954 1.24417509580164
2.5687428966418 1.26722145795548
2.58730541323742 1.28285985998207
2.62251700243816 1.29433042920734
2.64333416476756 1.33602361791541
2.67948897550178 1.38722348527647
2.72166591565624 1.42740486735385
2.75270055594358 1.43096683264484
2.80677818151326 1.46420167865521
2.85133018420882 1.4606499087354
2.91066751505617 1.4628090494307
2.98482763034345 1.45993833472835
3.06730554673034 1.46263587920374
3.14460274091814 1.44949469574389
3.23213784635088 1.44062697468932
3.31024163079453 1.4270307741753
3.3512951091394 1.40036671651812
3.4017711046021 1.39766894649338
3.38549056476237 1.37806342977231
3.40526244113241 1.37318389131059
3.40346612365705 1.36299155725777
3.39371821855194 1.33984612380685
3.4019140630963 1.32903653727561
3.43280327400255 1.31918825508543
3.42039131920034 1.266029771924
3.47478814252454 1.23864452174203
3.52481279222092 1.20708994254779
3.59465430557435 1.14070726337675
3.64292121266644 1.11078098661924
3.71732876891936 1.04934668163039
3.78228755694404 1.02317563752568
3.84326397997338 0.97866913059187
3.87591104971136 0.953033900190684
3.90045321168651 0.941730769001205
3.91996780654539 0.928809906030269
3.89384541236475 0.928975172026874
3.8532622045896 0.908870429954832
3.8009317601632 0.906522072719271
3.747730859615 0.906822278537671
3.66707106515983 0.907357408886252
3.5915272141181 0.883460231704356
3.52093959907854 0.878559911280428
3.45350962038186 0.871585647476596
};
% \addlegendentry{Ours}
\addplot [line width=1pt, color0]
table {%
2.73138986085617 0.657010612239058
2.75360432320259 0.645698437987604
2.7508083515257 0.646742571562861
2.74550851348316 0.62647268601071
2.72250258307611 0.615033248815969
2.70890036336189 0.587527391166454
2.70048674867281 0.566557237876796
2.6621245905157 0.56724183290176
2.65258940451437 0.562835575197254
2.65388347721636 0.574767195104584
2.67367372667819 0.569375858413319
2.71430448120537 0.580960908636404
2.75246716597602 0.589230026100572
2.86294371432932 0.578972956710099
2.90622962533318 0.602869530796653
2.95056109235385 0.610498545305097
2.99364341688218 0.592091640957174
3.02859427991752 0.596601918924841
3.05303250126545 0.605446191691559
3.07371619488321 0.59331040534939
3.13888316455779 0.578954124385501
3.16026821946876 0.593471293840019
3.2011036391208 0.587441829084113
3.26194031975455 0.585436550167668
3.324686196072 0.574030825320271
3.39168199789358 0.583491131606597
3.45507064740115 0.590701699692942
3.54791406710348 0.565351407396609
3.56893738355065 0.569375888805397
3.57555290050113 0.573217204811524
3.58155283205009 0.578697321920415
3.54932629113885 0.558774371932346
3.53567629037423 0.570017814051165
3.51997284555271 0.580211876341465
3.433437696447 0.601787538331989
3.39377508547388 0.616557406612546
3.35114383424233 0.606157718175345
3.31313908978661 0.603748215910125
3.28820382358359 0.612260202930852
3.27425116100906 0.623836672256871
3.21557335445532 0.639473359682488
3.09517642619145 0.656413354814575
3.0237912725378 0.671493474375941
2.96730721438741 0.660581288371215
2.88654480121457 0.651813349136982
2.7825827012005 0.619723430507855
2.66926498137833 0.625654022015665
2.56055966975768 0.616804803660629
2.49794002158032 0.633532465778361
2.46771011458673 0.618005370455619
2.41016471761844 0.622471582166816
2.38746546621496 0.648487353780215
2.38373945569784 0.682968405146507
2.37568340169178 0.685387413787086
2.37438529736967 0.701568477070616
2.39164826922535 0.729654784320017
2.3902769834158 0.736487016563697
2.38948524431167 0.735191718975739
2.40738441948655 0.747989026078135
2.45310103488526 0.757754302568014
2.49340311007651 0.787481070169994
2.55163154853127 0.808336627680076
2.69675335918421 0.837018512573694
2.7828881224921 0.857900350992185
2.8781491291644 0.87983859016243
2.97401096266729 0.914689697777957
3.04490491628471 0.91779790983678
3.10674838697937 0.942201302549024
3.14268939458707 0.96160500839244
3.19304735985892 0.968176824179276
3.21979241206349 0.977424816005104
3.23261212494025 0.98854923733403
3.24157911978149 0.997481256467301
3.25282331608796 0.999000764258679
3.27531500357294 1.00551834148556
3.30946525165874 1.00210401950882
3.42385911017909 1.00202748043467
3.4925721935755 0.991707550655818
3.55868134397623 0.999853118029554
3.62211398508616 0.987300409123901
3.65590555658562 0.980690779878946
3.66762449416404 1.00865384311342
3.65635034189895 1.00505626919742
3.57450225759951 0.964686392024289
3.5158561928853 0.975173104382569
3.41539104845262 0.992214323705194
3.33620951102076 0.977635694403429
3.25981144745224 0.970582182546276
3.21774691837508 0.98772491904037
3.18190880196593 1.00187251057426
3.17415752571927 1.04332747828965
3.17693561005654 1.08104896882526
3.22823553566057 1.13409488077488
3.23357894433589 1.12385764666774
3.25220577008086 1.14058092021073
3.2515280013004 1.13862285041618
3.20585824063552 1.12637073288414
3.06770239653192 1.11237674535651
2.97668730023826 1.12632378485632
2.84576909514051 1.15338153706751
2.72324522445048 1.1802201492966
2.66511587162346 1.189201715826
2.56737987444208 1.18631715643634
2.49471329396189 1.19710683876199
2.4093239167304 1.20630857760943
2.39956970376416 1.21285429981377
2.4376903406125 1.202070126601
2.44608059076592 1.23690657263644
2.49113634814668 1.22873410169901
2.49765126578515 1.24007702537664
2.57138202453032 1.22883324088849
2.60142040165522 1.27584502213182
2.63148326539495 1.30200693519575
2.65489646110252 1.35019264639585
2.67590307732644 1.41278413765946
2.71555056669599 1.46554881335009
2.75553028398983 1.48216535325547
2.80934333571462 1.49711376504688
2.92733741621492 1.48416807027805
3.00795400936487 1.48239981199108
3.113924435822 1.48464560222221
3.20209421874616 1.47546689225864
3.29513009591462 1.46906545974477
3.37406738163484 1.45005143552191
3.41678144100867 1.42274324602061
3.42748138373125 1.39132730307169
3.41629296783595 1.3824463086832
3.39991136029194 1.36938887207413
3.38655207560852 1.34900145876894
3.38100526590359 1.33633294363003
3.41160372311744 1.32677290340083
3.42411932536854 1.29090759232864
3.46911867279182 1.24151728469815
3.62774585499471 1.14207346885956
3.68700583597362 1.10617092039616
3.76279959859637 1.04095998209618
3.83677982126538 1.01456959616795
3.89950867841041 0.997756247245787
3.93350333458381 0.968176820352702
3.94612092052851 0.962598085536201
3.90038448028181 0.967805219897478
3.83280522309102 0.969189952480515
3.75225049030137 0.956281648576645
3.67462506650057 0.96179460005697
3.57868141193329 0.973224968241479
3.48884590654207 0.945283145524123
3.33868769525814 0.928901271267334
3.27961156151381 0.909942415671177
3.24219519876619 0.906760277506214
};
% \addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.79194092027163 0.675682647712128
% 2.79407119406988 0.703220041949035
% 2.79527527534208 0.711795270023535
% 2.79418461279521 0.726723723913668
% 2.7992917117979 0.727191847951841
% 2.81102871558341 0.713931684485897
% 2.79760860772589 0.702141990464947
% 2.78645569767935 0.677849089690324
% 2.75987040227934 0.655033487836737
% 2.74492820427677 0.622901863605389
% 2.73700166567946 0.58679370241161
% 2.71236227704775 0.564860313864813
% 2.68765841775157 0.564271594380181
% 2.67290493528827 0.559782760866558
% 2.66640708423765 0.565083992103844
% 2.67907644603627 0.555989880189345
% 2.71122620765581 0.563908618052208
% 2.73898108045827 0.569398247074381
% 2.78053817349636 0.560509803672526
% 2.83576546128013 0.56673625834506
% 2.86746986064176 0.591594042425316
% 2.90443960573929 0.60198713859095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.78004336357117 0.632818698883057
2.78473997116089 0.638318061828613
2.78169870376587 0.637591958045959
2.77279257774353 0.63290148973465
2.7611358165741 0.621461033821106
2.74732780456543 0.60774290561676
2.73093748092651 0.594337582588196
2.69390487670898 0.576365888118744
2.68285369873047 0.575522303581238
2.68129086494446 0.578539431095123
2.68994092941284 0.580935955047607
2.7073175907135 0.584364891052246
2.73254680633545 0.5893794298172
2.80578780174255 0.601789712905884
2.84787058830261 0.6033616065979
2.89023494720459 0.602049291133881
2.9271776676178 0.600774049758911
2.96092367172241 0.598361253738403
2.99176788330078 0.595715701580048
3.02260088920593 0.592634737491608
3.08351445198059 0.582817792892456
3.11538076400757 0.578564763069153
3.15450525283813 0.578361749649048
3.20232772827148 0.575249850749969
3.25803208351135 0.574694573879242
3.3161768913269 0.57064300775528
3.37219643592834 0.561338245868683
3.47152757644653 0.548518240451813
3.50878357887268 0.548225939273834
3.53404450416565 0.550397217273712
3.54474639892578 0.557612478733063
3.54177737236023 0.559260010719299
3.5278651714325 0.562194406986237
3.50693893432617 0.567442297935486
3.44325828552246 0.58589380979538
3.41175317764282 0.595011711120605
3.38133764266968 0.600455462932587
3.34080910682678 0.605159401893616
3.31128025054932 0.609150171279907
3.27819752693176 0.617089152336121
3.23718738555908 0.632509291172028
3.13333964347839 0.658334314823151
3.0713849067688 0.666970789432526
3.00010514259338 0.668299496173859
2.93614459037781 0.668152689933777
2.84673571586609 0.659588932991028
2.7660768032074 0.65624737739563
2.68826532363892 0.652865469455719
2.56908178329468 0.658845484256744
2.4967725276947 0.667507708072662
2.45544767379761 0.673418462276459
2.42531800270081 0.681628286838531
2.39972305297852 0.689211785793304
2.38822770118713 0.697850942611694
2.38112616539001 0.707625448703766
2.37244391441345 0.725314617156982
2.37436366081238 0.734794139862061
2.38197445869446 0.744607985019684
2.38410639762878 0.745479464530945
2.38410639762878 0.745479464530945
2.54188394546509 0.801227807998657
2.54188394546509 0.801227807998657
2.63489747047424 0.819602787494659
2.71523118019104 0.835769176483154
2.79587984085083 0.853483378887177
2.87371587753296 0.872008979320526
2.94537568092346 0.889821469783783
3.00989937782288 0.904130518436432
3.02894711494446 0.918487727642059
3.1410870552063 0.944109201431274
3.16888523101807 0.957380533218384
3.19266724586487 0.966566443443298
3.21331095695496 0.975494146347046
3.23522543907166 0.986978530883789
3.25612902641296 0.986358344554901
3.28694272041321 0.991490304470062
3.37403917312622 0.979946970939636
3.43747353553772 0.979255378246307
3.46730494499207 0.978964030742645
3.54685282707214 0.97417813539505
3.56150364875793 0.973176598548889
3.56150364875793 0.973176598548889
3.55420994758606 0.968668818473816
3.55420994758606 0.968668818473816
3.52897119522095 0.969216406345367
3.46123027801514 0.966148912906647
3.44793391227722 0.96590119600296
3.44793391227722 0.96590119600296
3.20479941368103 1.03704440593719
3.20479941368103 1.03704440593719
3.20333743095398 1.04014050960541
3.19610905647278 1.0569064617157
3.20433259010315 1.08610856533051
3.20877623558044 1.09527552127838
3.20877623558044 1.09527552127838
3.10875654220581 1.12826061248779
3.10875654220581 1.12826061248779
3.09200954437256 1.13175475597382
3.0337131023407 1.13904809951782
2.81984186172485 1.18516874313354
2.81984186172485 1.18516874313354
2.74672770500183 1.1967648267746
2.66049242019653 1.21030521392822
2.59113669395447 1.21736228466034
2.47602367401123 1.22587513923645
2.44892525672913 1.23063182830811
2.44124889373779 1.23750829696655
2.44737863540649 1.24806439876556
2.46477293968201 1.2597678899765
2.48559141159058 1.26518547534943
2.5109715461731 1.2717148065567
2.56022667884827 1.28673839569092
2.59123277664185 1.31957471370697
2.61795139312744 1.3553694486618
2.64434695243835 1.3904550075531
2.67542433738708 1.42694270610809
2.7141900062561 1.45624256134033
2.75917601585388 1.4771876335144
2.87690043449402 1.49541795253754
2.94824028015137 1.49557495117188
3.02909922599792 1.49183130264282
3.1125910282135 1.48014390468597
3.19374990463257 1.46717548370361
3.25704741477966 1.45282530784607
3.32147431373596 1.43851757049561
3.3886239528656 1.41326069831848
3.3969361782074 1.40173852443695
3.39630007743835 1.38950276374817
3.3953697681427 1.37267100811005
3.39798903465271 1.34983742237091
3.4073429107666 1.32186985015869
3.42936635017395 1.29361128807068
3.45953583717346 1.25897550582886
3.5581591129303 1.18452751636505
3.62155294418335 1.14020931720734
3.69111347198486 1.09253120422363
3.76070165634155 1.04756617546082
3.82333898544312 1.00902199745178
3.86648988723755 0.980598151683807
3.91346454620361 0.945891678333282
3.89978837966919 0.937991917133331
3.86199855804443 0.935832738876343
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
3.81219482421875 0.934732735157013
};
% \addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/XYZ_plot/YZ_plot_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

\definecolor{color0}{rgb}{1,0.188235294117647,0.188235294117647}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.97,0.03)},
  anchor=south east,
  draw=white!80!black
},
axis line style= {white},
tick align=outside,
tick pos=left,
% title={XY plot},
xmajorgrids,
xmajorticks=true,
xminorgrids,
xminorgrids=true,
ymajorgrids,
ymajorticks=true,
yminorgrids,
yminorgrids=true,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
            minor tick num = 3,
        minor grid style={dashed},
x grid style={white!69.0196078431373!black},
xmin=2.12877276002231, xmax=5.16023554096054,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymin=0.404950771684837, ymax=1.54912152663555,
ytick style={color=black}
]
\addplot [line width=1pt, color1]
table {%
2.2954216427211 0.456958533273505
2.31777733333452 0.49487950715315
2.33763132237825 0.529290846679961
2.37099891932597 0.558159603164172
2.39915270681096 0.581603031021609
2.43237971210357 0.611786834903712
2.48228843678183 0.619828840130322
2.50723591521166 0.618996725006725
2.57016757457341 0.628498933188615
2.61110224606921 0.618617386776924
2.65472841443386 0.614607834975727
2.69645540690029 0.595761471537237
2.73302168382298 0.587547656728352
2.78460398196515 0.590958649413665
2.83162000452564 0.591881436489796
2.87356750945619 0.587976674053637
2.92110874032325 0.602002696201986
2.97777074365821 0.60076945794349
3.02254324868717 0.599485724584289
3.09168373521269 0.606668274298737
3.13921476015578 0.601798888398763
3.20421169494298 0.601803934405946
3.26403626073103 0.624994661038883
3.308839878853 0.618054264314445
3.35316934072594 0.633184133508421
3.39633428969372 0.621581680741958
3.43829247711476 0.608653774943656
3.47959461117091 0.575099462250055
3.50625344126635 0.572568446543079
3.52119343091084 0.572684579097422
3.55705093628962 0.582454008587114
3.58359333367066 0.572830630436128
3.61456898100191 0.57180452551432
3.66382379414986 0.591655611703931
3.70350267599603 0.601012115979793
3.73986772656383 0.597981792655272
3.79459211832735 0.583684884156747
3.8589167167674 0.588966843957799
3.92124063459251 0.59836364931814
3.99992257838136 0.597582087944079
4.04932519277265 0.593434769797821
4.12635767857896 0.595421832362148
4.18267360064715 0.587168678823642
4.26760867678425 0.61323269863585
4.33154077984819 0.619632582003686
4.40008314812554 0.616422580950774
4.44440381051309 0.642036095741194
4.50073852441353 0.627756915178666
4.54387388862518 0.600471148141839
4.57784565316582 0.616949772980762
4.61861403199193 0.638238638834733
4.65154330276112 0.644806702267674
4.64713122150596 0.63367921735363
4.65879743126192 0.669634341593406
4.70050728512957 0.689264916110825
4.71491058954871 0.670265382912131
4.66791998111957 0.673432023045431
4.66456338564272 0.663546258504555
4.6514615485341 0.673433980979231
4.61419404518564 0.658970398827948
4.57197420706711 0.666703837043153
4.53758470508788 0.671934417412527
4.46912709671841 0.653844414067499
4.42916135383894 0.65968524912859
4.34431157821041 0.685358084016413
4.25510880352394 0.69307586205989
4.19943957942588 0.701937000010989
4.10868519659685 0.720095622449483
4.03084815122655 0.724435974931953
3.96403028690104 0.731778433289824
3.87862436703802 0.741309372872078
3.81631763394191 0.734836655091209
3.75911789075354 0.761445802916635
3.71140899378346 0.759670298112906
3.65434881455194 0.789383693822738
3.60680009805964 0.803059543989636
3.58652056216466 0.813322396882952
3.55043822523879 0.824897819019936
3.53340288012352 0.840585453207842
3.52469800454746 0.849309565324545
3.52613146215501 0.879255694390182
3.50699401464921 0.87885509882795
3.54187917205913 0.904607260521757
3.53992240245697 0.911776331357928
3.55999978636447 0.926187070720048
3.58142860940515 0.934689504021621
3.59744380239372 0.933546064274718
3.61509018467778 0.954467023878263
3.64513837855198 0.966678058414332
3.67737153279367 0.956835685894477
3.70888977791336 0.973457766206282
3.76111119411413 0.976457955699481
3.81567450582051 0.978880187295118
3.87873492581653 0.978734109121055
3.94845073923546 0.96995812975022
4.00428374323119 0.97968247290656
4.07382113314224 0.964835905435578
4.13568268890664 0.963451033157929
4.22094809638009 0.995157931634678
4.28045051725409 0.972477292621147
4.35828816630771 0.951715788645927
4.4285547032453 0.95058415575198
4.47791919068106 0.960707664166411
4.55688852191186 0.984419651304546
4.62122417091992 0.971751831612376
4.68121848605205 0.985980195289496
4.73146398329164 1.00240644796764
4.78350441257105 1.01293429952561
4.83617557570634 1.02839853580769
4.88170283359478 1.05042831139707
4.93427000544225 1.08165869271809
4.95618168663791 1.1164418127072
4.95904613541331 1.10544999991501
4.97156268814394 1.14284870029486
4.96111937046137 1.13248620425793
4.95360187519411 1.12856981396099
4.94110527615339 1.12136826430779
4.90874431955096 1.13975526380678
4.88445928190409 1.15118368116767
4.84402526283237 1.19951970322011
4.81363791051145 1.20221132249522
4.74639621909141 1.20186365755875
4.70270904061743 1.21033719632458
4.64008299046569 1.21925373592581
4.57376563144212 1.22002153597137
4.49753014236375 1.23972725018781
4.4323391667904 1.25168273938092
4.3752508721595 1.23057699533913
4.30350269834918 1.25793334385766
4.23780888271187 1.23861195945078
4.16120874459902 1.25862519873877
4.08395576213948 1.24417509580164
3.99330635987506 1.26722145795548
3.90717893497241 1.28285985998207
3.82396238528935 1.29433042920734
3.73051040945206 1.33602361791541
3.67380135412162 1.38722348527647
3.62732310185697 1.42740486735385
3.60816445200711 1.43096683264484
3.6098946166593 1.46420167865521
3.62974614417943 1.4606499087354
3.63564250016771 1.4628090494307
3.67777015015346 1.45993833472835
3.71591579123588 1.46263587920374
3.75898147583426 1.44949469574389
3.79552346889038 1.44062697468932
3.82217176546725 1.4270307741753
3.85307696350958 1.40036671651812
3.88682844445628 1.39766894649338
3.88813003946867 1.37806342977231
3.89499281734444 1.37318389131059
3.89927045065691 1.36299155725777
3.86211921707423 1.33984612380685
3.8675035459905 1.32903653727561
3.8550389843343 1.31918825508543
3.84582553031054 1.266029771924
3.82192860675603 1.23864452174203
3.8188104365502 1.20708994254779
3.81326090765918 1.14070726337675
3.79713954466694 1.11078098661924
3.77813464376112 1.04934668163039
3.76760799931913 1.02317563752568
3.73444576200688 0.97866913059187
3.70009956408722 0.953033900190684
3.64725299707619 0.941730769001205
3.57459200766659 0.928809906030269
3.49507137704457 0.928975172026874
3.40462543050264 0.908870429954832
3.31878053771735 0.906522072719271
3.21306244747252 0.906822278537671
3.11988218513941 0.907357408886252
3.03607055697764 0.883460231704356
2.95875103539358 0.878559911280428
2.90943214434925 0.871585647476596
};
% \addlegendentry{Ours }
\addplot [line width=1pt, color0]
table {%
2.26656652279223 0.657010612239058
2.35714382130048 0.645698437987604
2.46912835587662 0.646742571562861
2.54904439484317 0.62647268601071
2.61610617873149 0.615033248815969
2.67091839597072 0.587527391166454
2.71293841304514 0.566557237876796
2.8289300166783 0.56724183290176
2.8774984141375 0.562835575197254
2.9297412196155 0.574767195104584
2.99582687673874 0.569375858413319
3.04398971125765 0.580960908636404
3.11821334733149 0.589230026100572
3.23500900778058 0.578972956710099
3.29710121648793 0.602869530796653
3.34523716767429 0.610498545305097
3.38133012793502 0.592091640957174
3.42218117361351 0.596601918924841
3.46468232077013 0.605446191691559
3.50232048035524 0.59331040534939
3.53138675226301 0.578954124385501
3.56050365837881 0.593471293840019
3.5866636872793 0.587441829084113
3.61679437274807 0.585436550167668
3.66508438167831 0.574030825320271
3.71110243709038 0.583491131606597
3.74881729731915 0.590701699692942
3.87321212722207 0.565351407396609
3.94332451694098 0.569375888805397
4.02933308877975 0.573217204811524
4.09019776487595 0.578697321920415
4.16508434190537 0.558774371932346
4.22440220256894 0.570017814051165
4.30491172300629 0.580211876341465
4.45110679138145 0.601787538331989
4.49818151091311 0.616557406612546
4.54490620065661 0.606157718175345
4.58474715181891 0.603748215910125
4.61732776598191 0.612260202930852
4.64513056496436 0.623836672256871
4.68209119320882 0.639473359682488
4.67689255581475 0.656413354814575
4.71121890184527 0.671493474375941
4.72908747193449 0.660581288371215
4.68988240652772 0.651813349136982
4.67061365107596 0.619723430507855
4.66318354414061 0.625654022015665
4.62011394913901 0.616804803660629
4.52897023159987 0.633532465778361
4.45192419369431 0.618005370455619
4.40100904910164 0.622471582166816
4.31615609623814 0.648487353780215
4.22276895453488 0.682968405146507
4.1513383273049 0.685387413787086
4.06132088987714 0.701568477070616
3.91240201883462 0.729654784320017
3.83365064700832 0.736487016563697
3.76827987219866 0.735191718975739
3.71381407610171 0.747989026078135
3.67536896327288 0.757754302568014
3.62523566406642 0.787481070169994
3.57816940186485 0.808336627680076
3.53342552792813 0.837018512573694
3.51982087848909 0.857900350992185
3.51785614866331 0.87983859016243
3.52830366103386 0.914689697777957
3.51297702842778 0.91779790983678
3.54607893560372 0.942201302549024
3.56705205771726 0.96160500839244
3.60401281076548 0.968176824179276
3.62928634441175 0.977424816005104
3.64446115856433 0.98854923733403
3.67286715948425 0.997481256467301
3.71002245775272 0.999000764258679
3.74868867147703 1.00551834148556
3.80102292687833 1.00210401950882
3.93236281040655 1.00202748043467
4.00647533265346 0.991707550655818
4.06658877149959 0.999853118029554
4.13244637976297 0.987300409123901
4.1961475001081 0.980690779878946
4.27739257805573 1.00865384311342
4.34797240131824 1.00505626919742
4.49815402389132 0.964686392024289
4.55318674767089 0.975173104382569
4.63109920128498 0.992214323705194
4.70003778680557 0.977635694403429
4.76173411000382 0.970582182546276
4.80983644276065 0.98772491904037
4.85795678179988 1.00187251057426
4.94957756098052 1.04332747828965
5.00200282074395 1.08104896882526
5.02244177819062 1.13409488077488
5.01361867542625 1.12385764666774
5.01083580216477 1.14058092021073
4.99080038985157 1.13862285041618
4.97426244268442 1.12637073288414
4.92098387821703 1.11237674535651
4.89068955830255 1.12632378485632
4.85105684806315 1.15338153706751
4.81949275852938 1.1802201492966
4.75215494766644 1.189201715826
4.7000965492915 1.18631715643634
4.6370482848981 1.19710683876199
4.48600491487912 1.20630857760943
4.4143954307876 1.21285429981377
4.35508778149186 1.202070126601
4.28856147136882 1.23690657263644
4.21924292669192 1.22873410169901
4.14232480811796 1.24007702537664
4.05807420954335 1.22883324088849
3.87004989365037 1.27584502213182
3.78420504498652 1.30200693519575
3.69286429381683 1.35019264639585
3.63283440896259 1.41278413765946
3.60052766507381 1.46554881335009
3.59385470673663 1.48216535325547
3.61573660602321 1.49711376504688
3.67854550142618 1.48416807027805
3.72883539212453 1.48239981199108
3.78066445016795 1.48464560222221
3.82685738124627 1.47546689225864
3.86869615050429 1.46906545974477
3.89120954533684 1.45005143552191
3.91382799082125 1.42274324602061
3.9365317018496 1.39132730307169
3.93210645408647 1.3824463086832
3.93231502623131 1.36938887207413
3.89157036167549 1.34900145876894
3.87612959104443 1.33633294363003
3.86039258272765 1.32677290340083
3.84920205010396 1.29090759232864
3.82223804415004 1.24151728469815
3.81118702895529 1.14207346885956
3.78918835850452 1.10617092039616
3.76273740012428 1.04095998209618
3.74379930250183 1.01456959616795
3.71244778006224 0.997756247245787
3.66098633321622 0.968176820352702
3.51781356500873 0.962598085536201
3.42482929034603 0.967805219897478
3.32435618429358 0.969189952480515
3.22850809599341 0.956281648576645
3.12001769870334 0.96179460005697
3.02508054511676 0.973224968241479
2.9409249519996 0.945283145524123
2.83436894351627 0.928901271267334
2.79343853460443 0.909942415671177
2.76691028471854 0.906760277506214
};
% \addlegendentry{Point Cloud}
% \addplot [line width=1pt, green!50!black]
% table {%
% 2.35892892452518 0.675682647712128
% 2.42978630582589 0.703220041949035
% 2.48453329989567 0.711795270023535
% 2.53544276599431 0.726723723913668
% 2.60163917930246 0.727191847951841
% 2.63961579753378 0.713931684485897
% 2.70738974953776 0.702141990464947
% 2.75855673276656 0.677849089690324
% 2.8035775783111 0.655033487836737
% 2.84376380208128 0.622901863605389
% 2.8750528381069 0.58679370241161
% 2.92158934911775 0.564860313864813
% 2.97520109740467 0.564271594380181
% 3.02040086164092 0.559782760866558
% 3.06965739993503 0.565083992103844
% 3.13503458401981 0.555989880189345
% 3.1852448045617 0.563908618052208
% 3.26139294599305 0.569398247074381
% 3.31810043051243 0.560509803672526
% 3.38685611116533 0.56673625834506
% 3.45422213542551 0.591594042425316
% 3.50698442114095 0.60198713859095
% };
% \addlegendentry{Image}
\addplot [line width=1pt, black, dashed]
table {%
2.44961881637573 0.632818698883057
2.49184632301331 0.638318061828613
2.53642201423645 0.637591958045959
2.5811128616333 0.63290148973465
2.62548923492432 0.621461033821106
2.66858124732971 0.60774290561676
2.71244502067566 0.594337582588196
2.80324053764343 0.576365888118744
2.84974360466003 0.575522303581238
2.89853239059448 0.578539431095123
2.95167922973633 0.580935955047607
3.00733399391174 0.584364891052246
3.06419110298157 0.5893794298172
3.17853021621704 0.601789712905884
3.23518180847168 0.6033616065979
3.28984522819519 0.602049291133881
3.34109807014465 0.600774049758911
3.38540554046631 0.598361253738403
3.42358613014221 0.595715701580048
3.4562566280365 0.592634737491608
3.50875163078308 0.582817792892456
3.53420877456665 0.578564763069153
3.55867266654968 0.578361749649048
3.58785653114319 0.575249850749969
3.6181046962738 0.574694573879242
3.65492224693298 0.57064300775528
3.70083785057068 0.561338245868683
3.80997467041016 0.548518240451813
3.87289643287659 0.548225939273834
3.93877172470093 0.550397217273712
4.00425100326538 0.557612478733063
4.07564973831177 0.559260010719299
4.14390993118286 0.562194406986237
4.21157598495483 0.567442297935486
4.34743690490723 0.58589380979538
4.3992977142334 0.595011711120605
4.44696283340454 0.600455462932587
4.50991916656494 0.605159401893616
4.55272197723389 0.609150171279907
4.59152603149414 0.617089152336121
4.62049102783203 0.632509291172028
4.66143894195557 0.658334314823151
4.67684459686279 0.666970789432526
4.68613862991333 0.668299496173859
4.68156385421753 0.668152689933777
4.67292547225952 0.659588932991028
4.65167999267578 0.65624737739563
4.62711381912231 0.652865469455719
4.56195640563965 0.658845484256744
4.48921155929565 0.667507708072662
4.42907476425171 0.673418462276459
4.364417552948 0.681628286838531
4.28832912445068 0.689211785793304
4.21258687973022 0.697850942611694
4.13534498214722 0.707625448703766
3.9815731048584 0.725314617156982
3.91040086746216 0.734794139862061
3.84459114074707 0.744607985019684
3.83271741867065 0.745479464530945
3.83271741867065 0.745479464530945
3.59143424034119 0.801227807998657
3.59143424034119 0.801227807998657
3.55322051048279 0.819602787494659
3.53378105163574 0.835769176483154
3.52052617073059 0.853483378887177
3.51484632492065 0.872008979320526
3.51649236679077 0.889821469783783
3.52600789070129 0.904130518436432
3.53686928749084 0.918487727642059
3.56351637840271 0.944109201431274
3.57629799842834 0.957380533218384
3.59665036201477 0.966566443443298
3.62381148338318 0.975494146347046
3.65565609931946 0.986978530883789
3.696049451828 0.986358344554901
3.73732781410217 0.991490304470062
3.84776592254639 0.979946970939636
3.91309595108032 0.979255378246307
3.94392347335815 0.978964030742645
4.03354120254517 0.97417813539505
4.05302429199219 0.973176598548889
4.05302429199219 0.973176598548889
4.41191577911377 0.968668818473816
4.41191577911377 0.968668818473816
4.44498062133789 0.969216406345367
4.51591968536377 0.966148912906647
4.52946996688843 0.96590119600296
4.52946996688843 0.96590119600296
4.8422794342041 1.03704440593719
4.8422794342041 1.03704440593719
4.84621095657349 1.04014050960541
4.88337802886963 1.0569064617157
4.92765474319458 1.08610856533051
4.93645238876343 1.09527552127838
4.93645238876343 1.09527552127838
4.93231248855591 1.12826061248779
4.93231248855591 1.12826061248779
4.92480373382568 1.13175475597382
4.9000825881958 1.13904809951782
4.80996656417847 1.18516874313354
4.80996656417847 1.18516874313354
4.77510261535645 1.1967648267746
4.72225284576416 1.21030521392822
4.67178773880005 1.21736228466034
4.53933477401733 1.22587513923645
4.4741735458374 1.23063182830811
4.4066367149353 1.23750829696655
4.33526086807251 1.24806439876556
4.2646312713623 1.2597678899765
4.19270467758179 1.26518547534943
4.11613798141479 1.2717148065567
3.95782518386841 1.28673839569092
3.86118698120117 1.31957471370697
3.78020834922791 1.3553694486618
3.71509742736816 1.3904550075531
3.66681861877441 1.42694270610809
3.63695573806763 1.45624256134033
3.62501287460327 1.4771876335144
3.65587210655212 1.49541795253754
3.68864607810974 1.49557495117188
3.72396874427795 1.49183130264282
3.75977635383606 1.48014390468597
3.79366683959961 1.46717548370361
3.82296109199524 1.45282530784607
3.85447812080383 1.43851757049561
3.89113712310791 1.41326069831848
3.89532256126404 1.40173852443695
3.89313435554504 1.38950276374817
3.88669848442078 1.37267100811005
3.8734872341156 1.34983742237091
3.85793447494507 1.32186985015869
3.84170961380005 1.29361128807068
3.82747554779053 1.25897550582886
3.80352425575256 1.18452751636505
3.7911856174469 1.14020931720734
3.77538084983826 1.09253120422363
3.75537896156311 1.04756617546082
3.72709131240845 1.00902199745178
3.69070506095886 0.980598151683807
3.56822967529297 0.945891678333282
3.49198365211487 0.937991917133331
3.40586566925049 0.935832738876343
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
3.32272267341614 0.934732735157013
};
% \addlegendentry{GT}
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq1.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}

\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(-0.03,1.10)},
      anchor=north west,
      draw=white,
      /tikz/every even column/.append style={column sep=0.5cm},
    },
    legend columns=3,
    axis line style={white},
    tick align=outside,
    tick pos=left,
    % title={Seq 1 },
    x grid style={white!69.0196078431373!black},
    xmin=0.5, xmax=6.3,
    xtick style={color=black},
    xtick={1.4,3.4,5.4},
    xticklabels={X,Y,Z},
    y grid style={white!69.0196078431373!black},
    ylabel={ Error (m)},
    ymin=-0.0147050240191961, ymax=0.31,
    ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]

\draw[draw=color0,fill=color0, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color0,fill=color0,thick}
\addlegendentry{Tracking with only point cloud}

\draw[draw=color1,fill=color1, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color1,fill=color1,thick}
\addlegendentry{Tracking with only signal images}

\draw[draw=color2,fill=color2, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color2,fill=color2,thick}
\addlegendentry{Our approach}


\path [draw=color0, fill=color0]
(axis cs:0.9,0.0359016596706485)
--(axis cs:1.1,0.0359016596706485)
--(axis cs:1.1,0.123964853476531)
--(axis cs:0.9,0.123964853476531)
--(axis cs:0.9,0.0359016596706485)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0359016596706485
1 0.000594158118181198
};
\addplot [black, forget plot]
table {%
1 0.123964853476531
1 0.219165955456631
};
\addplot [black, forget plot]
table {%
0.95 0.000594158118181198
1.05 0.000594158118181198
};
\addplot [black, forget plot]
table {%
0.95 0.219165955456631
1.05 0.219165955456631
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0224564700129198)
--(axis cs:1.5,0.0224564700129198)
--(axis cs:1.5,0.131575909470591)
--(axis cs:1.3,0.131575909470591)
--(axis cs:1.3,0.0224564700129198)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0224564700129198
1.4 0.00368735991092217
};
\addplot [black, forget plot]
table {%
1.4 0.131575909470591
1.4 0.177035822042366
};
\addplot [black, forget plot]
table {%
1.35 0.00368735991092217
1.45 0.00368735991092217
};
\addplot [black, forget plot]
table {%
1.35 0.177035822042366
1.45 0.177035822042366
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.00882856225400375)
--(axis cs:1.9,0.00882856225400375)
--(axis cs:1.9,0.0287960855190496)
--(axis cs:1.7,0.0287960855190496)
--(axis cs:1.7,0.00882856225400375)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.00882856225400375
1.8 0.000267686459507033
};
\addplot [black, forget plot]
table {%
1.8 0.0287960855190496
1.8 0.0584475453119366
};
\addplot [black, forget plot]
table {%
1.75 0.000267686459507033
1.85 0.000267686459507033
};
\addplot [black, forget plot]
table {%
1.75 0.0584475453119366
1.85 0.0584475453119366
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0365788961205427)
--(axis cs:3.1,0.0365788961205427)
--(axis cs:3.1,0.0941762357336027)
--(axis cs:2.9,0.0941762357336027)
--(axis cs:2.9,0.0365788961205427)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0365788961205427
3 0.000869162330838336
};
\addplot [black, forget plot]
table {%
3 0.0941762357336027
3 0.17826472756505
};
\addplot [black, forget plot]
table {%
2.95 0.000869162330838336
3.05 0.000869162330838336
};
\addplot [black, forget plot]
table {%
2.95 0.17826472756505
3.05 0.17826472756505
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0936335797918026)
--(axis cs:3.5,0.0936335797918026)
--(axis cs:3.5,0.225292738533558)
--(axis cs:3.3,0.225292738533558)
--(axis cs:3.3,0.0936335797918026)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0936335797918026
3.4 0.00413021189512097
};
\addplot [black, forget plot]
table {%
3.4 0.225292738533558
3.4 0.294725109117304
};
\addplot [black, forget plot]
table {%
3.35 0.00413021189512097
3.45 0.00413021189512097
};
\addplot [black, forget plot]
table {%
3.35 0.294725109117304
3.45 0.294725109117304
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0105550124701859)
--(axis cs:3.9,0.0105550124701859)
--(axis cs:3.9,0.0439037283093395)
--(axis cs:3.7,0.0439037283093395)
--(axis cs:3.7,0.0105550124701859)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0105550124701859
3.8 0.000138631389560828
};
\addplot [black, forget plot]
table {%
3.8 0.0439037283093395
3.8 0.0823405821542753
};
\addplot [black, forget plot]
table {%
3.75 0.000138631389560828
3.85 0.000138631389560828
};
\addplot [black, forget plot]
table {%
3.75 0.0823405821542753
3.85 0.0823405821542753
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0255128619703696)
--(axis cs:5.1,0.0255128619703696)
--(axis cs:5.1,0.0756290965564553)
--(axis cs:4.9,0.0756290965564553)
--(axis cs:4.9,0.0255128619703696)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0255128619703696
5 0.00148441613567574
};
\addplot [black, forget plot]
table {%
5 0.0756290965564553
5 0.148283764805501
};
\addplot [black, forget plot]
table {%
4.95 0.00148441613567574
5.05 0.00148441613567574
};
\addplot [black, forget plot]
table {%
4.95 0.148283764805501
5.05 0.148283764805501
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.00532853403802855)
--(axis cs:5.5,0.00532853403802855)
--(axis cs:5.5,0.0127842448158017)
--(axis cs:5.3,0.0127842448158017)
--(axis cs:5.3,0.00532853403802855)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.00532853403802855
5.4 0.00142377354419265
};
\addplot [black, forget plot]
table {%
5.4 0.0127842448158017
5.4 0.0237795656365393
};
\addplot [black, forget plot]
table {%
5.35 0.00142377354419265
5.45 0.00142377354419265
};
\addplot [black, forget plot]
table {%
5.35 0.0237795656365393
5.45 0.0237795656365393
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.00727972918056854)
--(axis cs:5.9,0.00727972918056854)
--(axis cs:5.9,0.0231674857426256)
--(axis cs:5.7,0.0231674857426256)
--(axis cs:5.7,0.00727972918056854)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.00727972918056854
5.8 2.9744225399142e-05
};
\addplot [black, forget plot]
table {%
5.8 0.0231674857426256
5.8 0.0459741988826368
};
\addplot [black, forget plot]
table {%
5.75 2.9744225399142e-05
5.85 2.9744225399142e-05
};
\addplot [black, forget plot]
table {%
5.75 0.0459741988826368
5.85 0.0459741988826368
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0765784603353681
1.1 0.0765784603353681
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0798680383669237
1.5 0.0798680383669237
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.0167689702781684
1.9 0.0167689702781684
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0651368712573408
3.1 0.0651368712573408
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.167468870553379
3.5 0.167468870553379
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0247040115872634
3.9 0.0247040115872634
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0489386840818955
5.1 0.0489386840818955
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.00967427726703923
5.5 0.00967427726703923
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0139552293806988
5.9 0.0139552293806988
};
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq2.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=white!80!black
    },
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 2 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={ Error (m)},
ymin=-0.00876739680516033, ymax=0.184969536254822,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.00815245852515445)
--(axis cs:1.1,0.00815245852515445)
--(axis cs:1.1,0.0355660872611989)
--(axis cs:0.9,0.0355660872611989)
--(axis cs:0.9,0.00815245852515445)
--cycle;
\addplot [black, forget plot]
table {%
1 0.00815245852515445
1 0.000677464621831714
};
\addplot [black, forget plot]
table {%
1 0.0355660872611989
1 0.0760465676788473
};
\addplot [black, forget plot]
table {%
0.95 0.000677464621831714
1.05 0.000677464621831714
};
\addplot [black, forget plot]
table {%
0.95 0.0760465676788473
1.05 0.0760465676788473
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.00430830867868714)
--(axis cs:1.5,0.00430830867868714)
--(axis cs:1.5,0.0151839841291762)
--(axis cs:1.3,0.0151839841291762)
--(axis cs:1.3,0.00430830867868714)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.00430830867868714
1.4 0.0010557370823836
};
\addplot [black, forget plot]
table {%
1.4 0.0151839841291762
1.4 0.0231649600846127
};
\addplot [black, forget plot]
table {%
1.35 0.0010557370823836
1.45 0.0010557370823836
};
\addplot [black, forget plot]
table {%
1.35 0.0231649600846127
1.45 0.0231649600846127
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0108070949987866)
--(axis cs:1.9,0.0108070949987866)
--(axis cs:1.9,0.0469455026016019)
--(axis cs:1.7,0.0469455026016019)
--(axis cs:1.7,0.0108070949987866)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0108070949987866
1.8 3.88274248388498e-05
};
\addplot [black, forget plot]
table {%
1.8 0.0469455026016019
1.8 0.0722655397008891
};
\addplot [black, forget plot]
table {%
1.75 3.88274248388498e-05
1.85 3.88274248388498e-05
};
\addplot [black, forget plot]
table {%
1.75 0.0722655397008891
1.85 0.0722655397008891
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.00974226341835482)
--(axis cs:3.1,0.00974226341835482)
--(axis cs:3.1,0.0424458183453618)
--(axis cs:2.9,0.0424458183453618)
--(axis cs:2.9,0.00974226341835482)
--cycle;
\addplot [black, forget plot]
table {%
3 0.00974226341835482
3 0.0003648774884768
};
\addplot [black, forget plot]
table {%
3 0.0424458183453618
3 0.0759341926763533
};
\addplot [black, forget plot]
table {%
2.95 0.0003648774884768
3.05 0.0003648774884768
};
\addplot [black, forget plot]
table {%
2.95 0.0759341926763533
3.05 0.0759341926763533
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0336190006785358)
--(axis cs:3.5,0.0336190006785358)
--(axis cs:3.5,0.097577699413025)
--(axis cs:3.3,0.097577699413025)
--(axis cs:3.3,0.0336190006785358)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0336190006785358
3.4 0.0030644107688782
};
\addplot [black, forget plot]
table {%
3.4 0.097577699413025
3.4 0.176163312024822
};
\addplot [black, forget plot]
table {%
3.35 0.0030644107688782
3.45 0.0030644107688782
};
\addplot [black, forget plot]
table {%
3.35 0.176163312024822
3.45 0.176163312024822
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.00808186866347871)
--(axis cs:3.9,0.00808186866347871)
--(axis cs:3.9,0.0440748566983342)
--(axis cs:3.7,0.0440748566983342)
--(axis cs:3.7,0.00808186866347871)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.00808186866347871
3.8 0.0001008556550679
};
\addplot [black, forget plot]
table {%
3.8 0.0440748566983342
3.8 0.0881248202830607
};
\addplot [black, forget plot]
table {%
3.75 0.0001008556550679
3.85 0.0001008556550679
};
\addplot [black, forget plot]
table {%
3.75 0.0881248202830607
3.85 0.0881248202830607
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.00612243655419784)
--(axis cs:5.1,0.00612243655419784)
--(axis cs:5.1,0.0209237401912207)
--(axis cs:4.9,0.0209237401912207)
--(axis cs:4.9,0.00612243655419784)
--cycle;
\addplot [black, forget plot]
table {%
5 0.00612243655419784
5 0.000388261695153491
};
\addplot [black, forget plot]
table {%
5 0.0209237401912207
5 0.0392731995430584
};
\addplot [black, forget plot]
table {%
4.95 0.000388261695153491
5.05 0.000388261695153491
};
\addplot [black, forget plot]
table {%
4.95 0.0392731995430584
5.05 0.0392731995430584
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0139338719068252)
--(axis cs:5.5,0.0139338719068252)
--(axis cs:5.5,0.040402023571507)
--(axis cs:5.3,0.040402023571507)
--(axis cs:5.3,0.0139338719068252)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0139338719068252
5.4 0.00455167088083763
};
\addplot [black, forget plot]
table {%
5.4 0.040402023571507
5.4 0.065507495128893
};
\addplot [black, forget plot]
table {%
5.35 0.00455167088083763
5.45 0.00455167088083763
};
\addplot [black, forget plot]
table {%
5.35 0.065507495128893
5.45 0.065507495128893
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.004761184148176)
--(axis cs:5.9,0.004761184148176)
--(axis cs:5.9,0.0178303404227792)
--(axis cs:5.7,0.0178303404227792)
--(axis cs:5.7,0.004761184148176)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.004761184148176
5.8 0.000167742242199065
};
\addplot [black, forget plot]
table {%
5.8 0.0178303404227792
5.8 0.0364272724509153
};
\addplot [black, forget plot]
table {%
5.75 0.000167742242199065
5.85 0.000167742242199065
};
\addplot [black, forget plot]
table {%
5.75 0.0364272724509153
5.85 0.0364272724509153
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0202748343545978
1.1 0.0202748343545978
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.00982938124535071
1.5 0.00982938124535071
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.029147362000046
1.9 0.029147362000046
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0267552841689922
3.1 0.0267552841689922
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.0701316623582899
3.5 0.0701316623582899
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0192756859440788
3.9 0.0192756859440788
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0129318118170228
5.1 0.0129318118170228
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0231806449570045
5.5 0.0231806449570045
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0113959344884098
5.9 0.0113959344884098
};
\end{axis}

\end{tikzpicture}


==> tex/error_seq/error_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}


\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
    legend cell align={left},
    legend style={
      fill opacity=0.8,
      draw opacity=1,
      text opacity=1,
      at={(0.03,0.97)},
      anchor=north west,
      draw=white!80!black
    },
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 3 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={ Error (m)},
ymin=-0.00897775582982006, ymax=0.189937849485646,
ytick style={color=black},
        xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.0232780218577666)
--(axis cs:1.1,0.0232780218577666)
--(axis cs:1.1,0.0711417617143559)
--(axis cs:0.9,0.0711417617143559)
--(axis cs:0.9,0.0232780218577666)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0232780218577666
1 0.000596100612618056
};
\addplot [black, forget plot]
table {%
1 0.0711417617143559
1 0.142771459094593
};
\addplot [black, forget plot]
table {%
0.95 0.000596100612618056
1.05 0.000596100612618056
};
\addplot [black, forget plot]
table {%
0.95 0.142771459094593
1.05 0.142771459094593
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0088396449768362)
--(axis cs:1.5,0.0088396449768362)
--(axis cs:1.5,0.0177479663700559)
--(axis cs:1.3,0.0177479663700559)
--(axis cs:1.3,0.0088396449768362)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0088396449768362
1.4 0.000359157874370908
};
\addplot [black, forget plot]
table {%
1.4 0.0177479663700559
1.4 0.0278344120708334
};
\addplot [black, forget plot]
table {%
1.35 0.000359157874370908
1.45 0.000359157874370908
};
\addplot [black, forget plot]
table {%
1.35 0.0278344120708334
1.45 0.0278344120708334
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0114199810676545)
--(axis cs:1.9,0.0114199810676545)
--(axis cs:1.9,0.053081363686204)
--(axis cs:1.7,0.053081363686204)
--(axis cs:1.7,0.0114199810676545)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0114199810676545
1.8 0.000901600574375827
};
\addplot [black, forget plot]
table {%
1.8 0.053081363686204
1.8 0.108638698498432
};
\addplot [black, forget plot]
table {%
1.75 0.000901600574375827
1.85 0.000901600574375827
};
\addplot [black, forget plot]
table {%
1.75 0.108638698498432
1.85 0.108638698498432
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0279910207296199)
--(axis cs:3.1,0.0279910207296199)
--(axis cs:3.1,0.0771662866628215)
--(axis cs:2.9,0.0771662866628215)
--(axis cs:2.9,0.0279910207296199)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0279910207296199
3 0.000493392369484091
};
\addplot [black, forget plot]
table {%
3 0.0771662866628215
3 0.14312320811591
};
\addplot [black, forget plot]
table {%
2.95 0.000493392369484091
3.05 0.000493392369484091
};
\addplot [black, forget plot]
table {%
2.95 0.14312320811591
3.05 0.14312320811591
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.133592629973776)
--(axis cs:3.5,0.133592629973776)
--(axis cs:3.5,0.1742756192671)
--(axis cs:3.3,0.1742756192671)
--(axis cs:3.3,0.133592629973776)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.133592629973776
3.4 0.0787552872431321
};
\addplot [black, forget plot]
table {%
3.4 0.1742756192671
3.4 0.180896231062216
};
\addplot [black, forget plot]
table {%
3.35 0.0787552872431321
3.45 0.0787552872431321
};
\addplot [black, forget plot]
table {%
3.35 0.180896231062216
3.45 0.180896231062216
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0143334506366791)
--(axis cs:3.9,0.0143334506366791)
--(axis cs:3.9,0.0484907984263832)
--(axis cs:3.7,0.0484907984263832)
--(axis cs:3.7,0.0143334506366791)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0143334506366791
3.8 0.00152332401541067
};
\addplot [black, forget plot]
table {%
3.8 0.0484907984263832
3.8 0.0919856255534661
};
\addplot [black, forget plot]
table {%
3.75 0.00152332401541067
3.85 0.00152332401541067
};
\addplot [black, forget plot]
table {%
3.75 0.0919856255534661
3.85 0.0919856255534661
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.00718570042061395)
--(axis cs:5.1,0.00718570042061395)
--(axis cs:5.1,0.02510844997279)
--(axis cs:4.9,0.02510844997279)
--(axis cs:4.9,0.00718570042061395)
--cycle;
\addplot [black, forget plot]
table {%
5 0.00718570042061395
5 0.000149403716627639
};
\addplot [black, forget plot]
table {%
5 0.02510844997279
5 0.0515712221274507
};
\addplot [black, forget plot]
table {%
4.95 0.000149403716627639
5.05 0.000149403716627639
};
\addplot [black, forget plot]
table {%
4.95 0.0515712221274507
5.05 0.0515712221274507
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.016524061983732)
--(axis cs:5.5,0.016524061983732)
--(axis cs:5.5,0.0702343830365995)
--(axis cs:5.3,0.0702343830365995)
--(axis cs:5.3,0.016524061983732)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.016524061983732
5.4 0.00088228305353566
};
\addplot [black, forget plot]
table {%
5.4 0.0702343830365995
5.4 0.136660089747208
};
\addplot [black, forget plot]
table {%
5.35 0.00088228305353566
5.45 0.00088228305353566
};
\addplot [black, forget plot]
table {%
5.35 0.136660089747208
5.45 0.136660089747208
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.00499251809664381)
--(axis cs:5.9,0.00499251809664381)
--(axis cs:5.9,0.0189492854816761)
--(axis cs:5.7,0.0189492854816761)
--(axis cs:5.7,0.00499251809664381)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.00499251809664381
5.8 6.38625936102422e-05
};
\addplot [black, forget plot]
table {%
5.8 0.0189492854816761
5.8 0.0394391370956968
};
\addplot [black, forget plot]
table {%
5.75 6.38625936102422e-05
5.85 6.38625936102422e-05
};
\addplot [black, forget plot]
table {%
5.75 0.0394391370956968
5.85 0.0394391370956968
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.0452829561791654
1.1 0.0452829561791654
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0120809718295072
1.5 0.0120809718295072
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.0255258806510643
1.9 0.0255258806510643
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0515489334434402
3.1 0.0515489334434402
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.14480473897281
3.5 0.14480473897281
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.025519191420708
3.9 0.025519191420708
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0157743244749928
5.1 0.0157743244749928
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0370830731462402
5.5 0.0370830731462402
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.00942297550400267
5.9 0.00942297550400267
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq1.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(-0.03,1.12)},
  anchor=north west,
  draw=white,
/tikz/every even column/.append style={column sep=0.5cm},
},
legend columns = 3, 
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 1 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.034208951695738, ymax=0.721221921251871,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]

\draw[draw=color0,fill=color0, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color0,fill=color0,thick}
\addlegendentry{Tracking with only point cloud}

\draw[draw=color1,fill=color1, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color1,fill=color1,thick}
\addlegendentry{Tracking with only signal images}

\draw[draw=color2,fill=color2, thick] (axis cs:0,0) rectangle (axis cs:0,0);
\addlegendimage{ybar, ybar legend, draw=color2,fill=color2,thick}
\addlegendentry{Our approach}

\path [draw=color0, fill=color0]
(axis cs:0.9,0.109162671124885)
--(axis cs:1.1,0.109162671124885)
--(axis cs:1.1,0.344490432716165)
--(axis cs:0.9,0.344490432716165)
--(axis cs:0.9,0.109162671124885)
--cycle;
\addplot [black, forget plot]
table {%
1 0.109162671124885
1 0.000128815256426051
};
\addplot [black, forget plot]
table {%
1 0.344490432716165
1 0.686884154299707
};
\addplot [black, forget plot]
table {%
0.95 0.000128815256426051
1.05 0.000128815256426051
};
\addplot [black, forget plot]
table {%
0.95 0.686884154299707
1.05 0.686884154299707
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0919291443556336)
--(axis cs:1.5,0.0919291443556336)
--(axis cs:1.5,0.24845085936301)
--(axis cs:1.3,0.24845085936301)
--(axis cs:1.3,0.0919291443556336)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0919291443556336
1.4 0.00361160361343593
};
\addplot [black, forget plot]
table {%
1.4 0.24845085936301
1.4 0.392370148027017
};
\addplot [black, forget plot]
table {%
1.35 0.00361160361343593
1.45 0.00361160361343593
};
\addplot [black, forget plot]
table {%
1.35 0.392370148027017
1.45 0.392370148027017
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0651457039411474)
--(axis cs:1.9,0.0651457039411474)
--(axis cs:1.9,0.248436061039956)
--(axis cs:1.7,0.248436061039956)
--(axis cs:1.7,0.0651457039411474)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0651457039411474
1.8 0.0027373277432563
};
\addplot [black, forget plot]
table {%
1.8 0.248436061039956
1.8 0.493909091734377
};
\addplot [black, forget plot]
table {%
1.75 0.0027373277432563
1.85 0.0027373277432563
};
\addplot [black, forget plot]
table {%
1.75 0.493909091734377
1.85 0.493909091734377
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0771871383898404)
--(axis cs:3.1,0.0771871383898404)
--(axis cs:3.1,0.347491246148062)
--(axis cs:2.9,0.347491246148062)
--(axis cs:2.9,0.0771871383898404)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0771871383898404
3 0.000199890722223373
};
\addplot [black, forget plot]
table {%
3 0.347491246148062
3 0.677734254757247
};
\addplot [black, forget plot]
table {%
2.95 0.000199890722223373
3.05 0.000199890722223373
};
\addplot [black, forget plot]
table {%
2.95 0.677734254757247
3.05 0.677734254757247
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.158876445092808)
--(axis cs:3.5,0.158876445092808)
--(axis cs:3.5,0.366330405403881)
--(axis cs:3.3,0.366330405403881)
--(axis cs:3.3,0.158876445092808)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.158876445092808
3.4 0.0153142890715063
};
\addplot [black, forget plot]
table {%
3.4 0.366330405403881
3.4 0.486702403844719
};
\addplot [black, forget plot]
table {%
3.35 0.0153142890715063
3.45 0.0153142890715063
};
\addplot [black, forget plot]
table {%
3.35 0.486702403844719
3.45 0.486702403844719
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0411681137598663)
--(axis cs:3.9,0.0411681137598663)
--(axis cs:3.9,0.163136180242405)
--(axis cs:3.7,0.163136180242405)
--(axis cs:3.7,0.0411681137598663)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0411681137598663
3.8 0.000443114872510364
};
\addplot [black, forget plot]
table {%
3.8 0.163136180242405
3.8 0.342459269664861
};
\addplot [black, forget plot]
table {%
3.75 0.000443114872510364
3.85 0.000443114872510364
};
\addplot [black, forget plot]
table {%
3.75 0.342459269664861
3.85 0.342459269664861
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.070570502146341)
--(axis cs:5.1,0.070570502146341)
--(axis cs:5.1,0.276398234476372)
--(axis cs:4.9,0.276398234476372)
--(axis cs:4.9,0.070570502146341)
--cycle;
\addplot [black, forget plot]
table {%
5 0.070570502146341
5 0.000259953570465044
};
\addplot [black, forget plot]
table {%
5 0.276398234476372
5 0.531454865660448
};
\addplot [black, forget plot]
table {%
4.95 0.000259953570465044
5.05 0.000259953570465044
};
\addplot [black, forget plot]
table {%
4.95 0.531454865660448
5.05 0.531454865660448
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0136535369876245)
--(axis cs:5.5,0.0136535369876245)
--(axis cs:5.5,0.0975762615115577)
--(axis cs:5.3,0.0975762615115577)
--(axis cs:5.3,0.0136535369876245)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0136535369876245
5.4 0.00456348111469773
};
\addplot [black, forget plot]
table {%
5.4 0.0975762615115577
5.4 0.209099309075048
};
\addplot [black, forget plot]
table {%
5.35 0.00456348111469773
5.45 0.00456348111469773
};
\addplot [black, forget plot]
table {%
5.35 0.209099309075048
5.45 0.209099309075048
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.051383654669091)
--(axis cs:5.9,0.051383654669091)
--(axis cs:5.9,0.210674396423683)
--(axis cs:5.7,0.210674396423683)
--(axis cs:5.7,0.051383654669091)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.051383654669091
5.8 0.000249636769975581
};
\addplot [black, forget plot]
table {%
5.8 0.210674396423683
5.8 0.438200065621051
};
\addplot [black, forget plot]
table {%
5.75 0.000249636769975581
5.85 0.000249636769975581
};
\addplot [black, forget plot]
table {%
5.75 0.438200065621051
5.85 0.438200065621051
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.191737841303157
1.1 0.191737841303157
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.197800169460929
1.5 0.197800169460929
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.128881545706658
1.9 0.128881545706658
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.141984442865786
3.1 0.141984442865786
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.247618886526242
3.5 0.247618886526242
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0878626303248753
3.9 0.0878626303248753
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.134968087815255
5.1 0.134968087815255
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.0402095843975281
5.5 0.0402095843975281
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.105071468625511
5.9 0.105071468625511
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq2.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 2 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.0233556679147973, ymax=0.61,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.0454993116751612)
--(axis cs:1.1,0.0454993116751612)
--(axis cs:1.1,0.149575866732583)
--(axis cs:0.9,0.149575866732583)
--(axis cs:0.9,0.0454993116751612)
--cycle;
\addplot [black, forget plot]
table {%
1 0.0454993116751612
1 0.000176190755700745
};
\addplot [black, forget plot]
table {%
1 0.149575866732583
1 0.298551854208258
};
\addplot [black, forget plot]
table {%
0.95 0.000176190755700745
1.05 0.000176190755700745
};
\addplot [black, forget plot]
table {%
0.95 0.298551854208258
1.05 0.298551854208258
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0193088946071396)
--(axis cs:1.5,0.0193088946071396)
--(axis cs:1.5,0.0943910742063947)
--(axis cs:1.3,0.0943910742063947)
--(axis cs:1.3,0.0193088946071396)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0193088946071396
1.4 0.000377116058847271
};
\addplot [black, forget plot]
table {%
1.4 0.0943910742063947
1.4 0.132937731845124
};
\addplot [black, forget plot]
table {%
1.35 0.000377116058847271
1.45 0.000377116058847271
};
\addplot [black, forget plot]
table {%
1.35 0.132937731845124
1.45 0.132937731845124
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0512629607750226)
--(axis cs:1.9,0.0512629607750226)
--(axis cs:1.9,0.165225579088091)
--(axis cs:1.7,0.165225579088091)
--(axis cs:1.7,0.0512629607750226)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0512629607750226
1.8 0.00075650953687223
};
\addplot [black, forget plot]
table {%
1.8 0.165225579088091
1.8 0.332121025821897
};
\addplot [black, forget plot]
table {%
1.75 0.00075650953687223
1.85 0.00075650953687223
};
\addplot [black, forget plot]
table {%
1.75 0.332121025821897
1.85 0.332121025821897
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0417637473191679)
--(axis cs:3.1,0.0417637473191679)
--(axis cs:3.1,0.224785137712553)
--(axis cs:2.9,0.224785137712553)
--(axis cs:2.9,0.0417637473191679)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0417637473191679
3 0.000264292467084815
};
\addplot [black, forget plot]
table {%
3 0.224785137712553
3 0.470813364165661
};
\addplot [black, forget plot]
table {%
2.95 0.000264292467084815
3.05 0.000264292467084815
};
\addplot [black, forget plot]
table {%
2.95 0.470813364165661
3.05 0.470813364165661
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0448127976552481)
--(axis cs:3.5,0.0448127976552481)
--(axis cs:3.5,0.266378868864894)
--(axis cs:3.3,0.266378868864894)
--(axis cs:3.3,0.0448127976552481)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0448127976552481
3.4 0.00411012798469557
};
\addplot [black, forget plot]
table {%
3.4 0.266378868864894
3.4 0.456005566679127
};
\addplot [black, forget plot]
table {%
3.35 0.00411012798469557
3.45 0.00411012798469557
};
\addplot [black, forget plot]
table {%
3.35 0.456005566679127
3.45 0.456005566679127
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.032206746853467)
--(axis cs:3.9,0.032206746853467)
--(axis cs:3.9,0.147270781441821)
--(axis cs:3.7,0.147270781441821)
--(axis cs:3.7,0.032206746853467)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.032206746853467
3.8 0.00140957279476162
};
\addplot [black, forget plot]
table {%
3.8 0.147270781441821
3.8 0.285432958940515
};
\addplot [black, forget plot]
table {%
3.75 0.00140957279476162
3.85 0.00140957279476162
};
\addplot [black, forget plot]
table {%
3.75 0.285432958940515
3.85 0.285432958940515
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0365176475868445)
--(axis cs:5.1,0.0365176475868445)
--(axis cs:5.1,0.159425725571298)
--(axis cs:4.9,0.159425725571298)
--(axis cs:4.9,0.0365176475868445)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0365176475868445
5 0.00350969869741924
};
\addplot [black, forget plot]
table {%
5 0.159425725571298
5 0.341189883516642
};
\addplot [black, forget plot]
table {%
4.95 0.00350969869741924
5.05 0.00350969869741924
};
\addplot [black, forget plot]
table {%
4.95 0.341189883516642
5.05 0.341189883516642
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0352932972645825)
--(axis cs:5.5,0.0352932972645825)
--(axis cs:5.5,0.111943745306393)
--(axis cs:5.3,0.111943745306393)
--(axis cs:5.3,0.0352932972645825)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0352932972645825
5.4 0.000227750891903522
};
\addplot [black, forget plot]
table {%
5.4 0.111943745306393
5.4 0.195521128516952
};
\addplot [black, forget plot]
table {%
5.35 0.000227750891903522
5.45 0.000227750891903522
};
\addplot [black, forget plot]
table {%
5.35 0.195521128516952
5.45 0.195521128516952
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.0305767420525668)
--(axis cs:5.9,0.0305767420525668)
--(axis cs:5.9,0.172522100116694)
--(axis cs:5.7,0.172522100116694)
--(axis cs:5.7,0.0305767420525668)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.0305767420525668
5.8 0.00128623420413865
};
\addplot [black, forget plot]
table {%
5.8 0.172522100116694
5.8 0.369336006006802
};
\addplot [black, forget plot]
table {%
5.75 0.00128623420413865
5.85 0.00128623420413865
};
\addplot [black, forget plot]
table {%
5.75 0.369336006006802
5.85 0.369336006006802
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.100766256788645
1.1 0.100766256788645
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0682491611946423
1.5 0.0682491611946423
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.099464031339338
1.9 0.099464031339338
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.0989566119088892
3.1 0.0989566119088892
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.075984746026001
3.5 0.075984746026001
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.0908502564243308
3.9 0.0908502564243308
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0821778973760645
5.1 0.0821778973760645
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.079976425217278
5.5 0.079976425217278
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.0728472717659245
5.9 0.0728472717659245
};
\end{axis}

\end{tikzpicture}


==> tex/velo_error_seq/velo_error_seq3.tex <==
% This file was created with tikzplotlib v0.9.14.
\begin{tikzpicture}

% \definecolor{color0}{rgb}{0.6,0,0.980392156862745}
% \definecolor{color1}{rgb}{0.968627450980392,0.00784313725490196,0.164705882352941}
% \definecolor{color2}{rgb}{0.0235294117647059,0.32156862745098,1}
\definecolor{color0}{rgb}{0.90, 0.62, 0.00}
\definecolor{color1}{rgb}{0.34, 0.70, 0.91}
\definecolor{color2}{rgb}{0.00, 0.62, 0.45}
\definecolor{color3}{rgb}{0.94, 0.89, 0.27}
\definecolor{color4}{rgb}{0.00, 0.45, 0.69}
\definecolor{color5}{rgb}{0.83, 0.37, 0.00}

\begin{axis}[
    width=\figurewidth,
    height=\figureheight,
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
axis line style={white},
tick align=outside,
tick pos=left,
% title={Seq 3 },
x grid style={white!69.0196078431373!black},
xmin=0.5, xmax=6.3,
xtick style={color=black},
xtick={1.4,3.4,5.4},
xticklabels={X,Y,Z},
y grid style={white!69.0196078431373!black},
ylabel={Velocity Error (m/s)},
ymin=-0.0375045054404742, ymax=0.78781873238659,
ytick style={color=black},
    xmajorgrids,
    % xmajorticks=true,
    % xmin=-0.5, xmax=3.3125,
    xminorgrids,
    ymajorgrids,
    ymajorticks=true,
    minor y tick num = 3,
    minor y grid style={dashed},
    yminorgrids,
    yticklabel style={
            /pgf/number format/fixed,
            /pgf/number format/precision=5
    },
    scaled y ticks=false,
]
\path [draw=color0, fill=color0]
(axis cs:0.9,0.050925850163972)
--(axis cs:1.1,0.050925850163972)
--(axis cs:1.1,0.305209551337428)
--(axis cs:0.9,0.305209551337428)
--(axis cs:0.9,0.050925850163972)
--cycle;
\addplot [black, forget plot]
table {%
1 0.050925850163972
1 0.000915280434687915
};
\addplot [black, forget plot]
table {%
1 0.305209551337428
1 0.658851716939473
};
\addplot [black, forget plot]
table {%
0.95 0.000915280434687915
1.05 0.000915280434687915
};
\addplot [black, forget plot]
table {%
0.95 0.658851716939473
1.05 0.658851716939473
};
\path [draw=color1, fill=color1]
(axis cs:1.3,0.0186842481424454)
--(axis cs:1.5,0.0186842481424454)
--(axis cs:1.5,0.103976060431693)
--(axis cs:1.3,0.103976060431693)
--(axis cs:1.3,0.0186842481424454)
--cycle;
\addplot [black, forget plot]
table {%
1.4 0.0186842481424454
1.4 0.000318754243475716
};
\addplot [black, forget plot]
table {%
1.4 0.103976060431693
1.4 0.180866270180915
};
\addplot [black, forget plot]
table {%
1.35 0.000318754243475716
1.45 0.000318754243475716
};
\addplot [black, forget plot]
table {%
1.35 0.180866270180915
1.45 0.180866270180915
};
\path [draw=color2, fill=color2]
(axis cs:1.7,0.0607938102103689)
--(axis cs:1.9,0.0607938102103689)
--(axis cs:1.9,0.255498452503433)
--(axis cs:1.7,0.255498452503433)
--(axis cs:1.7,0.0607938102103689)
--cycle;
\addplot [black, forget plot]
table {%
1.8 0.0607938102103689
1.8 0.000215207845459808
};
\addplot [black, forget plot]
table {%
1.8 0.255498452503433
1.8 0.509395351885571
};
\addplot [black, forget plot]
table {%
1.75 0.000215207845459808
1.85 0.000215207845459808
};
\addplot [black, forget plot]
table {%
1.75 0.509395351885571
1.85 0.509395351885571
};
\path [draw=color0, fill=color0]
(axis cs:2.9,0.0540813292258191)
--(axis cs:3.1,0.0540813292258191)
--(axis cs:3.1,0.234681439454613)
--(axis cs:2.9,0.234681439454613)
--(axis cs:2.9,0.0540813292258191)
--cycle;
\addplot [black, forget plot]
table {%
3 0.0540813292258191
3 0.00025457195519607
};
\addplot [black, forget plot]
table {%
3 0.234681439454613
3 0.50483313777927
};
\addplot [black, forget plot]
table {%
2.95 0.00025457195519607
3.05 0.00025457195519607
};
\addplot [black, forget plot]
table {%
2.95 0.50483313777927
3.05 0.50483313777927
};
\path [draw=color1, fill=color1]
(axis cs:3.3,0.0341207415404121)
--(axis cs:3.5,0.0341207415404121)
--(axis cs:3.5,0.341801049261369)
--(axis cs:3.3,0.341801049261369)
--(axis cs:3.3,0.0341207415404121)
--cycle;
\addplot [black, forget plot]
table {%
3.4 0.0341207415404121
3.4 0.00729099756574314
};
\addplot [black, forget plot]
table {%
3.4 0.341801049261369
3.4 0.750304039758087
};
\addplot [black, forget plot]
table {%
3.35 0.00729099756574314
3.45 0.00729099756574314
};
\addplot [black, forget plot]
table {%
3.35 0.750304039758087
3.45 0.750304039758087
};
\path [draw=color2, fill=color2]
(axis cs:3.7,0.0470434830938093)
--(axis cs:3.9,0.0470434830938093)
--(axis cs:3.9,0.190534730347155)
--(axis cs:3.7,0.190534730347155)
--(axis cs:3.7,0.0470434830938093)
--cycle;
\addplot [black, forget plot]
table {%
3.8 0.0470434830938093
3.8 0.000923772653984578
};
\addplot [black, forget plot]
table {%
3.8 0.190534730347155
3.8 0.397895565899473
};
\addplot [black, forget plot]
table {%
3.75 0.000923772653984578
3.85 0.000923772653984578
};
\addplot [black, forget plot]
table {%
3.75 0.397895565899473
3.85 0.397895565899473
};
\path [draw=color0, fill=color0]
(axis cs:4.9,0.0370850724055838)
--(axis cs:5.1,0.0370850724055838)
--(axis cs:5.1,0.144242538996679)
--(axis cs:4.9,0.144242538996679)
--(axis cs:4.9,0.0370850724055838)
--cycle;
\addplot [black, forget plot]
table {%
5 0.0370850724055838
5 1.01871880286986e-05
};
\addplot [black, forget plot]
table {%
5 0.144242538996679
5 0.29127738534024
};
\addplot [black, forget plot]
table {%
4.95 1.01871880286986e-05
5.05 1.01871880286986e-05
};
\addplot [black, forget plot]
table {%
4.95 0.29127738534024
5.05 0.29127738534024
};
\path [draw=color1, fill=color1]
(axis cs:5.3,0.0345189067087442)
--(axis cs:5.5,0.0345189067087442)
--(axis cs:5.5,0.216801981745139)
--(axis cs:5.3,0.216801981745139)
--(axis cs:5.3,0.0345189067087442)
--cycle;
\addplot [black, forget plot]
table {%
5.4 0.0345189067087442
5.4 0.00468124038173312
};
\addplot [black, forget plot]
table {%
5.4 0.216801981745139
5.4 0.421482532405152
};
\addplot [black, forget plot]
table {%
5.35 0.00468124038173312
5.45 0.00468124038173312
};
\addplot [black, forget plot]
table {%
5.35 0.421482532405152
5.45 0.421482532405152
};
\path [draw=color2, fill=color2]
(axis cs:5.7,0.0333654972375574)
--(axis cs:5.9,0.0333654972375574)
--(axis cs:5.9,0.145628655344953)
--(axis cs:5.7,0.145628655344953)
--(axis cs:5.7,0.0333654972375574)
--cycle;
\addplot [black, forget plot]
table {%
5.8 0.0333654972375574
5.8 0.000549304948028739
};
\addplot [black, forget plot]
table {%
5.8 0.145628655344953
5.8 0.312894917001754
};
\addplot [black, forget plot]
table {%
5.75 0.000549304948028739
5.85 0.000549304948028739
};
\addplot [black, forget plot]
table {%
5.75 0.312894917001754
5.85 0.312894917001754
};
\addplot [line width=1pt, white, forget plot]
table {%
0.9 0.129738371745527
1.1 0.129738371745527
};
\addplot [line width=1pt, white, forget plot]
table {%
1.3 0.0536968219671419
1.5 0.0536968219671419
};
\addplot [line width=1pt, white, forget plot]
table {%
1.7 0.107509878653638
1.9 0.107509878653638
};
\addplot [line width=1pt, white, forget plot]
table {%
2.9 0.121060592272317
3.1 0.121060592272317
};
\addplot [line width=1pt, white, forget plot]
table {%
3.3 0.109664642493887
3.5 0.109664642493887
};
\addplot [line width=1pt, white, forget plot]
table {%
3.7 0.119131419941609
3.9 0.119131419941609
};
\addplot [line width=1pt, white, forget plot]
table {%
4.9 0.0768678127111805
5.1 0.0768678127111805
};
\addplot [line width=1pt, white, forget plot]
table {%
5.3 0.115904482344118
5.5 0.115904482344118
};
\addplot [line width=1pt, white, forget plot]
table {%
5.7 0.083997795576003
5.9 0.083997795576003
};
\end{axis}

\end{tikzpicture}

